Investigating Length Issues in Document-level Machine Translation

Transformer architectures are increasingly effective at processing and generating very long chunks of texts, opening new perspectives for document-level machine translation (MT). In this work, we challenge the ability of MT systems to handle texts comprising up to several thousands of tokens. We design and implement a new approach designed to precisely measure the effect of length increments on MT outputs. Our experiments with two representative architectures unambiguously show that (a)~translation performance decreases with the length of the input text; (b)~the position of sentences within the document matters, and translation quality is higher for sentences occurring earlier in a document. We further show that manipulating the distribution of document lengths and of positional embeddings only marginally mitigates such problems. Our results suggest that even though document-level MT is computationally feasible, it does not yet match the performance of sentence-based MT.

==> tabs/comet-sent/res-nllb-TED-distill-testsets-comet.tex <==

\begin{table}
  \centering
    \scalebox{0.72}{

    \begin{tabular}{llrrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 0.84 & 0.85 & 0.85 & 0.84 \\
     & Unif.\ & 0.82 & 0.84 & 0.84 & 0.83 \\
      \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 0.81 & 0.82 & 0.82 & 0.81 \\
     & Unif.\ & 0.81 & 0.82 & 0.82 & 0.81 \\
      \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 0.81 & 0.82 & 0.81 & 0.80 \\
     & Unif.\ & 0.81 & 0.82 & 0.81 & 0.81 \\
      \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 0.69 & 0.69 & 0.70 & 0.69 \\
     & Unif.\ & 0.74 & 0.75 & 0.74 & 0.73 \\
      \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 0.58 & 0.59 & 0.60 & 0.58 \\
     & Unif.\ & 0.67 & 0.65 & 0.67 & 0.67 \\
      \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 0.56 & 0.56 & 0.55 & 0.53 \\
     & Unif.\ & 0.61 & 0.65 & 0.62 & 0.60 \\
      \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 0.50 & 0.49 & 0.49 & 0.49 \\
     & Unif.\ & 0.55 & 0.58 & 0.54 & 0.56 \\
      \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 0.47 & 0.42 & 0.48 & 0.45 \\
     & Unif.\ & 0.51 & 0.49 & 0.51 & 0.48 \\
     \bottomrule
    \end{tabular}

}
  \caption{COMET for \FTnllbII (FT.\ ), \UNIFnllbII (Unif.\ ) trained on \tedII with target max source document length 2048 }
  \label{tab:res-nllb-comet-ted-distill}
\end{table}

==> tabs/comet-sent/res-nllb-TED-unif-testsets-comet.tex <==

\begin{table}
  \centering
    \scalebox{0.72}{

    \begin{tabular}{llrrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 0.84 & 0.85 & 0.85 & 0.84 \\
     & Unif.\ & 0.82 & 0.83 & 0.83 & 0.83 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 0.80 & 0.81 & 0.81 & 0.81 \\
     & Unif.\ & 0.80 & 0.81 & 0.81 & 0.81 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 0.80 & 0.81 & 0.81 & 0.81 \\
     & Unif.\ & 0.81 & 0.82 & 0.81 & 0.81 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 0.80 & 0.81 & 0.81 & 0.81 \\
     & Unif.\ & 0.81 & 0.82 & 0.82 & 0.81 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 0.78 & 0.79 & 0.78 & 0.78 \\
     & Unif.\ & 0.80 & 0.81 & 0.81 & 0.80 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 0.71 & 0.73 & 0.70 & 0.69 \\
     & Unif.\ & 0.76 & 0.79 & 0.76 & 0.75 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 0.61 & 0.60 & 0.61 & 0.60 \\
     & Unif.\ & 0.62 & 0.61 & 0.61 & 0.64 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 0.57 & 0.53 & 0.57 & 0.54 \\
     & Unif.\ & 0.59 & 0.57 & 0.57 & 0.54 \\
     \bottomrule
    \end{tabular}

}
  \caption{COMET for \FTnllbI (FT.\ ),  \UNIFnllbI (Unif.\ ) trained on \tedI with target max source document length 2048 }
  \label{tab:res-nllb-comet-ted-unif}
\end{table}

==> tabs/comet-sent/res-tower-TED-distill-testsets-comet.tex <==
\begin{table}
  \centering
    \scalebox{0.72}{
    \begin{tabular}{llrrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 0.85 & 0.86 & 0.85 & 0.85 \\
     & Unif.\ & 0.85 & 0.86 & 0.85 & 0.85 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 0.83 & 0.84 & 0.83 & 0.83 \\
     & Unif.\ & 0.83 & 0.84 & 0.83 & 0.83 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 0.82 & 0.84 & 0.83 & 0.82 \\
     & Unif.\ & 0.82 & 0.84 & 0.83 & 0.82 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 0.82 & 0.83 & 0.83 & 0.82 \\
     & Unif.\ & 0.82 & 0.83 & 0.83 & 0.82 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 0.81 & 0.81 & 0.82 & 0.81 \\
     & Unif.\ & 0.81 & 0.82 & 0.83 & 0.81 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 0.78 & 0.82 & 0.81 & 0.81 \\
     & Unif.\ & 0.78 & 0.82 & 0.81 & 0.81 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 0.80 & 0.79 & 0.79 & 0.80 \\
     & Unif.\ & 0.79 & 0.78 & 0.79 & 0.78 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 0.68 & 0.69 & 0.68 & 0.64 \\
     & Unif.\ & 0.69 & 0.70 & 0.70 & 0.62 \\
     \bottomrule
    \end{tabular}
    }
  \caption{COMET score for \FTtowerII (FT.\ ),  \UNIFtowerII (Unif.\ ) trained on \tedII with target max source document length 2048 ($M = 4096$). }
  \label{tab:res-tower-comet-ted-distill}
\end{table}


==> tabs/comet-sent/res-tower-TED-unif-testsets-comet.tex <==
\begin{table}
  \centering
    \scalebox{0.72}{
    
    \begin{tabular}{llrrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 0.85 & 0.86 & 0.85 & 0.85 \\
     & Unif.\ & 0.85 & 0.86 & 0.85 & 0.85 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 0.83 & 0.84 & 0.83 & 0.83 \\
     & Unif.\ & 0.83 & 0.84 & 0.83 & 0.82 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 0.82 & 0.84 & 0.83 & 0.82 \\
     & Unif.\ & 0.82 & 0.84 & 0.83 & 0.82 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 0.82 & 0.83 & 0.83 & 0.82 \\
     & Unif.\ & 0.82 & 0.84 & 0.83 & 0.82 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 0.81 & 0.81 & 0.83 & 0.81 \\
     & Unif.\ & 0.81 & 0.83 & 0.83 & 0.81 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 0.80 & 0.82 & 0.81 & 0.81 \\
     & Unif.\ & 0.80 & 0.82 & 0.81 & 0.81 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 0.79 & 0.79 & 0.80 & 0.80 \\
     & Unif.\ & 0.80 & 0.80 & 0.78 & 0.79 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 0.68 & 0.72 & 0.69 & 0.64 \\
     & Unif.\ & 0.70 & 0.72 & 0.69 & 0.67 \\
     \bottomrule
    \end{tabular}

    }
  \caption{COMET score for \FTtowerI(FT.\ ),  \UNIFtowerI (Unif.\ ) trained on \tedI with target max source document length 2048 ($M = 4096$). }
  \label{tab:res-tower-comet-ted-unif}
\end{table}


==> tabs/comet-sent/ttest-by-block-all.tex <==

\begin{table} %[h]
    \centering
    % \begin{minipage}{0.46\textwidth}
    \scalebox{0.65}{
    \begin{tabular}{rrrrrr}
    \toprule
     & \multicolumn{1}{c}{\model{NLLB}} & \multicolumn{1}{c}{FT-U} & \multicolumn{1}{c}{Unif-U} & \multicolumn{1}{c}{FT-G} & \multicolumn{1}{c}{Unif-G} \\
     \midrule
    sent-256 & 9.2 \footnotesize{(0.00)} & 0.8 \footnotesize{(0.00)} & -2.1 \footnotesize{(0.00)} & 0.4 \footnotesize{(0.03)} & -0.7 \footnotesize{(0.00)} \\
    256-512 & 19.1 \footnotesize{(0.00)} & - & -0.4 \footnotesize{(0.03)} & - & - \\
    512-768 & 6.9 \footnotesize{(0.00)} & - & -0.6 \footnotesize{(0.00)} & 5.9 \footnotesize{(0.00)} & 2.5 \footnotesize{(0.00)} \\
    768-1024 & - & 0.5 \footnotesize{(0.01)} & - & 7.2 \footnotesize{(0.00)} & 3.0 \footnotesize{(0.00)} \\
    1024-1200 & nan & 3.5 \footnotesize{(0.00)} & 1.9 \footnotesize{(0.00)} & 4.0 \footnotesize{(0.00)} & 3.3 \footnotesize{(0.00)} \\
    1200-1600 & nan & 6.8 \footnotesize{(0.00)} & 6.5 \footnotesize{(0.00)} & 5.8 \footnotesize{(0.00)} & 5.5 \footnotesize{(0.00)} \\
    1600-2048 & nan & 5.2 \footnotesize{(0.00)} & 4.5 \footnotesize{(0.00)} & 4.2 \footnotesize{(0.00)} & 5.7 \footnotesize{(0.00)} \\
     \midrule
    sent-256 & 16.7 \footnotesize{(0.00)} & 3.5 \footnotesize{(0.00)} & 1.7 \footnotesize{(0.00)} & 2.7 \footnotesize{(0.00)} & 2.1 \footnotesize{(0.00)} \\
    256-512 & 20.7 \footnotesize{(0.00)} & - & -0.4 \footnotesize{(0.03)} & 0.6 \footnotesize{(0.00)} & - \\
    512-768 & 5.6 \footnotesize{(0.00)} & - & - & 11.6 \footnotesize{(0.00)} & 7.2 \footnotesize{(0.00)} \\
    768-1024 & 5.2 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} & 0.8 \footnotesize{(0.04)} & 10.4 \footnotesize{(0.00)} & 7.6 \footnotesize{(0.00)} \\
    1024-1200 & nan & 7.4 \footnotesize{(0.00)} & 4.3 \footnotesize{(0.00)} & 3.8 \footnotesize{(0.00)} & 4.7 \footnotesize{(0.00)} \\
    1200-1600 & nan & 9.6 \footnotesize{(0.00)} & 13.4 \footnotesize{(0.00)} & 5.4 \footnotesize{(0.00)} & 5.5 \footnotesize{(0.00)} \\
    1600-2048 & nan & 5.1 \footnotesize{(0.00)} & 5.0 \footnotesize{(0.00)} & 3.9 \footnotesize{(0.00)} & 5.6 \footnotesize{(0.00)} \\
    \bottomrule
    \end{tabular}
    }   
    % \caption{Average differences (and p-values) evaluated on \textbf{ds-BLEU} for full TED talks (top) and on $100\times$\textbf{COMET} for realigned sentences (bottom), for \model{NLLB} models. Only p-values $< 0.05$ are reported. D1 and D2 denote \tedI and \tedII respectively. }
    % \label{tab:ttest-by-block-nllb}
    % \end{minipage}%
    % \hspace{0.02\textwidth} % Space between tables
    \medskip
    % \begin{minipage}{0.46\textwidth}
    \scalebox{0.65}{
    \begin{tabular}{rrrrrr}
    \toprule
     & \model{Tower} & FT-U & Unif-U & FT-G & Unif-G \\
     \midrule
    sent-256 & - & - & - & - & - \\
    256-512 & - & 0.9 \footnotesize{(0.02)} & 0.8 \footnotesize{(0.05)} & 0.6 \footnotesize{(0.00)} & 0.6 \footnotesize{(0.00)} \\
    512-768 & - & - & - & 0.6 \footnotesize{(0.04)} & - \\
    768-1024 & 3.4 \footnotesize{(0.00)} & - & 1.0 \footnotesize{(0.05)} & 1.7 \footnotesize{(0.01)} & 1.2 \footnotesize{(0.01)} \\
    1024-1200 & - & - & - & - & - \\
    1200-1600 & 4.7 \footnotesize{(0.00)} & 1.7 \footnotesize{(0.01)} & 2.1 \footnotesize{(0.01)} & 1.6 \footnotesize{(0.02)} & 2.0 \footnotesize{(0.01)} \\
    1600-2048 & 5.9 \footnotesize{(0.00)} & 7.5 \footnotesize{(0.00)} & 6.5 \footnotesize{(0.00)} & 8.1 \footnotesize{(0.00)} & 7.8 \footnotesize{(0.00)} \\
     \midrule
    sent-256 & 3.9 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} & 2.4 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} \\
    256-512 & - & 0.4 \footnotesize{(0.02)} & - & 0.2 \footnotesize{(0.03)} & 0.3 \footnotesize{(0.02)} \\
    512-768 & - & - & - & 0.3 \footnotesize{(0.00)} & - \\
    768-1024 & 2.9 \footnotesize{(0.00)} & 1.0 \footnotesize{(0.04)} & 0.5 \footnotesize{(0.00)} & 1.1 \footnotesize{(0.03)} & 0.8 \footnotesize{(0.00)} \\
    1024-1200 & - & - & 1.0 \footnotesize{(0.03)} & - & - \\
    1200-1600 & 6.2 \footnotesize{(0.00)} & 1.7 \footnotesize{(0.00)} & 1.8 \footnotesize{(0.02)} & - & 1.9 \footnotesize{(0.01)} \\
    1600-2048 & 8.7 \footnotesize{(0.00)} & 10.0 \footnotesize{(0.00)} & 8.9 \footnotesize{(0.00)} & 11.0 \footnotesize{(0.00)} & 10.2 \footnotesize{(0.00)} \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Average differences (and p-values) evaluated on \textbf{ds-BLEU} (top) of full TED talks and on $100\times$\textbf{COMET} (bottom) of realigned parallel sentences, for \model{NLLB} (left) and \model{TowerBase} (right) models. - for p-values $> 0.05$. U and G respectively denote \tedI and \tedII. `nan' marks no translated test sets. }

    \label{tab:ttest-by-block}
    % \end{minipage}
\end{table}



==> tabs/other-format/data-stat-testsets.tex <==

\begin{table}
  \centering

    \scalebox{0.8}{
    \begin{tabular}{l|rr|rr|rr}
    \toprule
     & \multicolumn{2}{r|}{\corpus{TED-full}} & \multicolumn{2}{r|}{\tedII} & \multicolumn{2}{r}{\tedI} \\
     % \midrule
     & train & dev & train & dev & train & dev \\
     \midrule
    count & 1831 & 19 & 15625 & 160 & 10582 & 106 \\
    mean & 2915 & 2861 & 341 & 339 & 504 & 512 \\
    min & 56 & 680 & 3 & 12 & 3 & 42 \\
    max & 8706 & 6076 & 1022 & 959 & 1020 & 991 \\
    \bottomrule
    \end{tabular}
    }

    \bigskip
  
\setlength{\tabcolsep}{2pt}
  \scalebox{0.82}{
    \begin{tabular}{lrrrrrrrr}
    \toprule
     & \multicolumn{2}{r}{2014} & \multicolumn{2}{r}{2015} & \multicolumn{2}{r}{2016} & \multicolumn{2}{r}{2017} \\
     \midrule
     $l_{max}$ & count & mean & count & mean & count & mean & count & mean \\
     \midrule
    sent & 1335 & 23 & 1104 & 23 & 1185 & 24 & 1479 & 23 \\
    256 & 129 & 234 & 107 & 234 & 123 & 232 & 144 & 234 \\
    512 & 68 & 443 & 56 & 447 & 63 & 454 & 74 & 456 \\
    768 & 48 & 628 & 40 & 626 & 45 & 635 & 51 & 662 \\
    1024 & 37 & 815 & 30 & 835 & 35 & 817 & 40 & 844 \\
    1200 & 32 & 942 & 26 & 963 & 31 & 922 & 34 & 992 \\
    1600 & 26 & 1160 & 24 & 1043 & 23 & 1243 & 27 & 1250 \\
    2048 & 20 & 1507 & 16 & 1565 & 21 & 1361 & 23 & 1467 \\
    doc & 15 & 2010 & 12 & 2086 & 13 & 2199 & 12 & 2812 \\
    \bottomrule
    \end{tabular}
    
}
  \caption{Top: Statistics of TEDTalks. 
  % All lengths in English \model{NLLB} pieces.
  Bottom: Statistics of the test-sets based on TED talks from IWSLT \testset{tst2014}, \testset{tst2015}, \testset{tst2016} and \testset{tst2017}. 'count' denotes the number of parallel pseudo-documents, 'mean' denotes the average length of source (i.e.\ English) pseudo-documents. All lengths are counted in pieces using \model{NLLB} tokenizer.}
  \label{tab:data-stat}
\end{table}


==> tabs/other-format/data-stat-train-dev.tex <==
\begin{table}
  \centering
    \scalebox{0.8}{
    \begin{tabular}{l|rr|rr|rr}
    \toprule
     & \multicolumn{2}{r|}{\corpus{TED-full}} & \multicolumn{2}{r|}{\corpus{TED-distill}} & \multicolumn{2}{r}{\corpus{TED-unif}} \\
     % \midrule
     & train & dev & train & dev & train & dev \\
     \midrule
    count & 1831 & 19 & 15625 & 160 & 10582 & 106 \\
    mean & 2915 & 2861 & 341 & 339 & 504 & 512 \\
    min & 56 & 680 & 3 & 12 & 3 & 42 \\
    max & 8706 & 6076 & 1022 & 959 & 1020 & 991 \\
    \bottomrule
    \end{tabular}}
    
  \caption{Statistics of TEDTalks. All lengths in English \model{NLLB} pieces.}
  \label{tab:data-train}
\end{table}

% \begin{table}
%   \centering
%     \scalebox{0.8}{

%     }  \caption{Data stat TED en}
%   \label{tab:data-train}
% \end{table}

==> tabs/other-format/res-base-nllb200-bleu-comet.tex <==
\begin{table}
  \centering
    \scalebox{0.82}{
    \begin{tabular}{l|rrrr}
    \toprule
    $l_{max}$ & 2014 & 2015 & 2016 & 2017 \\
    \midrule
    sent & 42.8 \footnotesize{(0.98)} & 41.2 \footnotesize{(1.0)} & 39.7 \footnotesize{(1.0)} & 39.1 \footnotesize{(1.0)} \\
    256 & 31.1 \footnotesize{(0.82)} & 31.6 \footnotesize{(0.84)} & 30.4 \footnotesize{(0.86)} & 29.5 \footnotesize{(0.86)} \\
    512 & 12.3 \footnotesize{(0.47)} & 12.7 \footnotesize{(0.6)} & 11.2 \footnotesize{(0.53)} & 10.8 \footnotesize{(0.49)} \\
    768 & 6.1 \footnotesize{(0.28)} & 6.7 \footnotesize{(0.34)} & 7.0 \footnotesize{(0.52)} & 5.2 \footnotesize{(0.26)} \\
    1024 & 5.7 \footnotesize{(0.66)} & 5.3 \footnotesize{(0.54)} & 4.6 \footnotesize{(0.59)} & 4.4 \footnotesize{(0.55)} \\
    \bottomrule
    \end{tabular}
}

    \medskip

    % \scalebox{0.9}{
    \begin{tabular}{l|rrrr}
    \toprule
     & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    sent & 0.84 & 0.85 & 0.85 & 0.84 \\
    256 & 0.68 & 0.69 & 0.68 & 0.66 \\
    512 & 0.49 & 0.47 & 0.47 & 0.46 \\
    768 & 0.43 & 0.42 & 0.40 & 0.41 \\
    1024 & 0.36 & 0.37 & 0.36 & 0.36 \\
    \bottomrule
    \end{tabular}
    
% }
  \caption{BLEU (top) and COMET (bottom) scores evaluated on translations using \model{NLLB200-distilled-600M}. }
  \label{tab:res-base-nllb}
\end{table}

==> tabs/other-format/res-base-towerbase-bleu-comet.tex <==


\begin{table}
  \centering

    \scalebox{0.82}{
    % prompt English $SRC\nFrench:
    \begin{tabular}{l|rrrr}
    \toprule
     $l_{max}$ & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    sent & 41.3 \footnotesize{(1.0)} & 39.8 \footnotesize{(1.0)} & 37.7 \footnotesize{(1.0)} & 35.0 \footnotesize{(1.0)} \\
    256 & 40.9 \footnotesize{(0.96)} & 39.9 \footnotesize{(1.0)} & 38.7 \footnotesize{(1.0)} & 36.2 \footnotesize{(1.0)} \\
    512 & 39.6 \footnotesize{(0.99)} & 35.7 \footnotesize{(1.0)} & 37.6 \footnotesize{(1.0)} & 37.5 \footnotesize{(1.0)} \\
    768 & 36.5 \footnotesize{(1.0)} & 36.2 \footnotesize{(1.0)} & 36.1 \footnotesize{(1.0)} & 36.7 \footnotesize{(1.0)} \\
    1024 & 34.8 \footnotesize{(1.0)} & 28.2 \footnotesize{(1.0)} & 31.8 \footnotesize{(1.0)} & 32.0 \footnotesize{(1.0)} \\
    1200 & 34.0 \footnotesize{(0.98)} & 31.4 \footnotesize{(1.0)} & 33.1 \footnotesize{(1.0)} & 32.3 \footnotesize{(1.0)} \\
    1600 & 28.5 \footnotesize{(1.0)} & 31.2 \footnotesize{(1.0)} & 21.5 \footnotesize{(1.0)} & 27.1 \footnotesize{(1.0)} \\
    2048 & 15.4 \footnotesize{(1.0)} & 24.3 \footnotesize{(1.0)} & 22.2 \footnotesize{(1.0)} & 19.7 \footnotesize{(0.96)} \\
    \bottomrule
    \end{tabular}
     }

    \medskip

    \centering
    \scalebox{0.7}{
    \begin{tabular}{l|rrrr}
    \toprule
     & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    sent & 0.84 & 0.85 & 0.85 & 0.85 \\
    256 & 0.80 & 0.81 & 0.82 & 0.80 \\
    512 & 0.79 & 0.80 & 0.82 & 0.80 \\
    768 & 0.78 & 0.78 & 0.80 & 0.80 \\
    1024 & 0.76 & 0.73 & 0.78 & 0.76 \\
    1200 & 0.73 & 0.74 & 0.77 & 0.76 \\
    1600 & 0.70 & 0.72 & 0.65 & 0.68 \\
    2048 & 0.52 & 0.63 & 0.65 & 0.57 \\
    \bottomrule
    \end{tabular}
    }
   
  \caption{BLEU (top) and COMET (bottom) scores evaluated on translations using \model{TowerBase-7b}. }
  \label{tab:res-base-tower}
\end{table}



==> tabs/other-format/res-tower-TED-distill-testsets-vanilla-bleu.tex <==
\begin{table}
  \centering
    \scalebox{0.7}{
    
\begin{tabular}{llllll}
\toprule
 &  & 2014 & 2015 & 2016 & 2017 \\
 \midrule
\multirow[c]{2}{*}{sent} & FT.\ & 43.8 \footnotesize{(0.99)} & 41.7 \footnotesize{(1.0)} & 40.4 \footnotesize{(1.0)} & 36.8 \footnotesize{(1.0)} \\
 & Unif.\ & 43.8 \footnotesize{(0.99)} & 41.6 \footnotesize{(1.0)} & 40.4 \footnotesize{(1.0)} & 37.3 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{256} & FT.\ & 41.8 \footnotesize{(1.0)} & 41.5 \footnotesize{(1.0)} & 40.0 \footnotesize{(1.0)} & 38.8 \footnotesize{(1.0)} \\
 & Unif.\ & 41.6 \footnotesize{(1.0)} & 41.5 \footnotesize{(1.0)} & 40.0 \footnotesize{(1.0)} & 38.8 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{512} & FT.\ & 41.2 \footnotesize{(1.0)} & 41.5 \footnotesize{(1.0)} & 39.2 \footnotesize{(1.0)} & 38.5 \footnotesize{(1.0)} \\
 & Unif.\ & 41.1 \footnotesize{(1.0)} & 41.3 \footnotesize{(1.0)} & 39.2 \footnotesize{(1.0)} & 38.2 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{768} & FT.\ & 41.4 \footnotesize{(1.0)} & 40.9 \footnotesize{(1.0)} & 37.6 \footnotesize{(1.0)} & 37.6 \footnotesize{(1.0)} \\
 & Unif.\ & 41.4 \footnotesize{(1.0)} & 40.8 \footnotesize{(1.0)} & 37.5 \footnotesize{(1.0)} & 37.2 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1024} & FT.\ & 39.4 \footnotesize{(1.0)} & 36.4 \footnotesize{(1.0)} & 35.6 \footnotesize{(1.0)} & 37.1 \footnotesize{(1.0)} \\
 & Unif.\ & 39.2 \footnotesize{(1.0)} & 39.2 \footnotesize{(1.0)} & 36.5 \footnotesize{(1.0)} & 36.8 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1200} & FT.\ & 38.3 \footnotesize{(1.0)} & 39.7 \footnotesize{(1.0)} & 36.1 \footnotesize{(1.0)} & 37.4 \footnotesize{(1.0)} \\
 & Unif.\ & 38.3 \footnotesize{(1.0)} & 39.4 \footnotesize{(1.0)} & 36.5 \footnotesize{(1.0)} & 37.1 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1600} & FT.\ & 39.1 \footnotesize{(1.0)} & 37.7 \footnotesize{(1.0)} & 33.4 \footnotesize{(1.0)} & 35.1 \footnotesize{(1.0)} \\
 & Unif.\ & 39.3 \footnotesize{(1.0)} & 36.6 \footnotesize{(1.0)} & 34.0 \footnotesize{(1.0)} & 33.7 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{2048} & FT.\ & 26.8 \footnotesize{(1.0)} & 27.6 \footnotesize{(1.0)} & 27.3 \footnotesize{(1.0)} & 24.7 \footnotesize{(1.0)} \\
 & Unif.\ & 27.4 \footnotesize{(1.0)} & 29.0 \footnotesize{(1.0)} & 28.8 \footnotesize{(1.0)} & 22.9 \footnotesize{(1.0)} \\
 \bottomrule
\end{tabular}

    }
  \caption{BLEU for \FTtowerII (FT.\ ) and \UNIFtowerII (Unif-full) trained on \tedII with target max source document length 2048 ($M = 4096$). }
  \label{tab:res-tower-bleu-ted-distill}
\end{table}


==> tabs/other-format/res-tower-TED-unif-testsets-vanilla-bleu.tex <==
\begin{table}
  \centering
    \scalebox{0.7}{

\begin{tabular}{llllll}
\toprule
 &  & 2014 & 2015 & 2016 & 2017 \\
 \midrule
\multirow[c]{2}{*}{sent} & FT.\ & 43.5 \footnotesize{(0.99)} & 41.8 \footnotesize{(1.0)} & 40.3 \footnotesize{(1.0)} & 36.7 \footnotesize{(1.0)} \\
 & Unif.\ & 43.6 \footnotesize{(0.99)} & 41.7 \footnotesize{(1.0)} & 40.4 \footnotesize{(1.0)} & 36.7 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{256} & FT.\ & 43.5 \footnotesize{(0.99)} & 41.5 \footnotesize{(1.0)} & 40.0 \footnotesize{(1.0)} & 38.7 \footnotesize{(1.0)} \\
 & Unif.\ & 41.8 \footnotesize{(1.0)} & 41.6 \footnotesize{(1.0)} & 40.1 \footnotesize{(1.0)} & 38.8 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{512} & FT.\ & 40.3 \footnotesize{(1.0)} & 41.5 \footnotesize{(1.0)} & 39.0 \footnotesize{(1.0)} & 38.3 \footnotesize{(1.0)} \\
 & Unif.\ & 38.9 \footnotesize{(1.0)} & 41.6 \footnotesize{(1.0)} & 39.2 \footnotesize{(1.0)} & 38.5 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{768} & FT.\ & 41.6 \footnotesize{(1.0)} & 41.1 \footnotesize{(1.0)} & 39.1 \footnotesize{(1.0)} & 37.6 \footnotesize{(1.0)} \\
 & Unif.\ & 40.4 \footnotesize{(1.0)} & 41.2 \footnotesize{(1.0)} & 39.3 \footnotesize{(1.0)} & 37.8 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1024} & FT.\ & 40.9 \footnotesize{(0.99)} & 37.7 \footnotesize{(1.0)} & 36.8 \footnotesize{(1.0)} & 36.4 \footnotesize{(1.0)} \\
 & Unif.\ & 39.6 \footnotesize{(1.0)} & 40.5 \footnotesize{(1.0)} & 36.8 \footnotesize{(1.0)} & 36.1 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1200} & FT.\ & 40.0 \footnotesize{(1.0)} & 39.5 \footnotesize{(1.0)} & 36.9 \footnotesize{(1.0)} & 37.5 \footnotesize{(1.0)} \\
 & Unif.\ & 39.7 \footnotesize{(1.0)} & 39.8 \footnotesize{(1.0)} & 35.9 \footnotesize{(1.0)} & 37.6 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1600} & FT.\ & 38.6 \footnotesize{(0.97)} & 37.4 \footnotesize{(1.0)} & 34.1 \footnotesize{(1.0)} & 36.4 \footnotesize{(1.0)} \\
 & Unif.\ & 38.4 \footnotesize{(1.0)} & 38.3 \footnotesize{(1.0)} & 32.9 \footnotesize{(1.0)} & 34.3 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{2048} & FT.\ & 29.4 \footnotesize{(1.0)} & 31.3 \footnotesize{(1.0)} & 27.2 \footnotesize{(1.0)} & 25.3 \footnotesize{(1.0)} \\
 & Unif.\ & 30.0 \footnotesize{(1.0)} & 31.8 \footnotesize{(1.0)} & 26.4 \footnotesize{(1.0)} & 27.8 \footnotesize{(1.0)} \\
 \bottomrule
\end{tabular}

}

  \caption{BLEU for \FTtowerI (FT.\ ), \UNIFtowerI (Unif.\ ) trained on \tedI with target max source document length 2048 ($M = 4096$).}
  \label{tab:res-tower-bleu-ted-unif}
\end{table}


==> tabs/other-format/stat-no-repetition-nllb.tex <==



\begin{table}
  \centering
    \scalebox{0.7}{

    \begin{tabular}{lrrrrlll}
    \toprule
     & 256 & 512 & 768 & 1024 & 1200 & 1600 & 2048 \\
     \midrule
    NLLB & 0.96 & 0.65 & 0.51 & 0.34 & - & - & - \\
    FT-D1 & 0.99 & 0.97 & 0.92 & 0.91 & 0.87 & 0.74 & 0.56 \\
    % Unif-r7-D1 & 0.99 & 0.95 & 0.92 & 0.75 & 0.67 & 0.59 & 0.54 \\
    Unif-D1 & 0.99 & 0.97 & 0.93 & 0.90 & 0.80 & 0.66 & 0.68 \\
    FT-D2 & 0.99 & 0.97 & 0.89 & 0.69 & 0.60 & 0.43 & 0.31 \\
    % Unif-r7-D2 & 0.98 & 0.95 & 0.79 & 0.78 & 0.70 & 0.68 & 0.57 \\
    Unif-D2 & 0.99 & 0.96 & 0.84 & 0.80 & 0.73 & 0.75 & 0.64 \\
    \bottomrule
    \end{tabular}
    }  
    \caption{Percentage of pseudo-documents among \testset{tst2014}, \testset{tst2015}, \testset{tst2016} and \testset{tst2017} in which no $10$gram repetition is detected from the translation given by NLLB-based models.}
  \label{tab:stat-no-repeat-nllb}
\end{table}

==> tabs/other-format/stat-no-repetition-tower.tex <==
\begin{table}
  \centering
    \scalebox{0.7}{
    \begin{tabular}{lrrrrrrr}
    \toprule
     & 256 & 512 & 768 & 1024 & 1200 & 1600 & 2048 \\
     \midrule
    Tower & 0.99 & 0.95 & 0.82 & 0.75 & 0.70 & 0.64 & 0.45 \\
    FT-D1 & 0.99 & 0.95 & 0.90 & 0.85 & 0.87 & 0.77 & 0.41 \\
    % Unif-r7-D1 & 0.99 & 0.95 & 0.91 & 0.85 & 0.89 & 0.76 & 0.40 \\
    Unif-D1 & 0.98 & 0.95 & 0.91 & 0.85 & 0.84 & 0.72 & 0.39 \\
    FT-D2 & 0.98 & 0.95 & 0.90 & 0.85 & 0.81 & 0.74 & 0.38 \\
    % Unif-r7-D2 & 0.98 & 0.93 & 0.91 & 0.85 & 0.80 & 0.66 & 0.39 \\
    Unif-D2 & 0.98 & 0.93 & 0.90 & 0.84 & 0.80 & 0.72 & 0.36 \\
    \bottomrule
    \end{tabular}

    }  
    \caption{Percentage of pseudo-documents among \testset{tst2014}, \testset{tst2015}, \testset{tst2016} and \testset{tst2017} in which no $10$gram repetition is detected from the translation given by \model{TowerBase}-based models.}
  \label{tab:stat-no-repeat-tower}
\end{table}

==> tabs/res-nllb-TED-distill-testsets-ds-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}
        \scalebox{0.72}{
        \begin{tabular}{rl|rrrr}
        \toprule
         &  & 2014 & 2015 & 2016 & 2017 \\
         \midrule
        \multirow[c]{2}{*}{sent} & FT & 43.8 \footnotesize{(0.98)} & 44.0 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.00)} & 41.3 \footnotesize{(1.00)} \\
         & Unif & 42.4 \footnotesize{(0.98)} & 42.5 \footnotesize{(0.99)} & 39.7 \footnotesize{(1.00)} & 40.2 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{256} & FT & 43.5 \footnotesize{(0.98)} & 43.1 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.00)} & 40.8 \footnotesize{(1.00)} \\
         & Unif & 43.9 \footnotesize{(0.98)} & 43.2 \footnotesize{(0.99)} & 39.7 \footnotesize{(1.00)} & 40.6 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{512} & FT & 43.5 \footnotesize{(0.98)} & 43.4 \footnotesize{(0.98)} & 40.2 \footnotesize{(1.00)} & 40.4 \footnotesize{(1.00)} \\
         & Unif & 43.8 \footnotesize{(0.98)} & 43.8 \footnotesize{(0.99)} & 39.8 \footnotesize{(1.00)} & 41.0 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{768} & FT & 36.6 \footnotesize{(0.87)} & 36.4 \footnotesize{(0.88)} & 35.3 \footnotesize{(0.92)} & 35.6 \footnotesize{(0.93)} \\
         & Unif & 41.8 \footnotesize{(0.95)} & 39.1 \footnotesize{(0.88)} & 38.1 \footnotesize{(0.95)} & 39.4 \footnotesize{(0.97)} \\
         \midrule
        \multirow[c]{2}{*}{1024} & FT & 28.6 \footnotesize{(0.70)} & 29.1 \footnotesize{(0.75)} & 28.9 \footnotesize{(0.80)} & 28.7 \footnotesize{(0.79)} \\
         & Unif & 36.1 \footnotesize{(0.81)} & 38.7 \footnotesize{(0.87)} & 34.9 \footnotesize{(0.87)} & 37.2 \footnotesize{(0.92)} \\
         \midrule
        \multirow[c]{2}{*}{1200} & FT & 25.2 \footnotesize{(0.64)} & 25.8 \footnotesize{(0.74)} & 24.1 \footnotesize{(0.71)} & 24.3 \footnotesize{(0.73)} \\
         & Unif & 34.6 \footnotesize{(0.80)} & 36.4 \footnotesize{(0.82)} & 30.0 \footnotesize{(0.74)} & 32.4 \footnotesize{(0.80)} \\
         \midrule
        \multirow[c]{2}{*}{1600} & FT & 18.2 \footnotesize{(0.53)} & 19.3 \footnotesize{(0.62)} & 19.2 \footnotesize{(0.62)} & 19.6 \footnotesize{(0.59)} \\
         & Unif & 25.5 \footnotesize{(0.59)} & 30.1 \footnotesize{(0.70)} & 26.9 \footnotesize{(0.68)} & 29.4 \footnotesize{(0.72)} \\
         \midrule
        \multirow[c]{2}{*}{2048} & FT & 15.4 \footnotesize{(0.49)} & 12.4 \footnotesize{(0.52)} & 16.7 \footnotesize{(0.58)} & 14.8 \footnotesize{(0.61)} \\
         & Unif & 22.0 \footnotesize{(0.51)} & 21.6 \footnotesize{(0.50)} & 24.3 \footnotesize{(0.60)} & 20.6 \footnotesize{(0.53)} \\
         \bottomrule
        \end{tabular}
        }
 
    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}

    \scalebox{0.72}{

    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT & 84 & 85 & 85 & 84 \\
     & Unif & 82 & 84 & 84 & 83 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT & 81 & 82 & 82 & 81 \\
     & Unif & 81 & 82 & 82 & 81 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT & 81 & 82 & 81 & 80 \\
     & Unif & 81 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT & 69 & 69 & 70 & 69 \\
     & Unif & 74 & 75 & 74 & 73 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT & 58 & 59 & 60 & 58 \\
     & Unif & 67 & 65 & 67 & 67 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT & 56 & 56 & 55 & 53 \\
     & Unif & 61 & 65 & 62 & 60 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT & 50 & 49 & 49 & 49 \\
     & Unif & 55 & 58 & 54 & 56 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT & 47 & 42 & 48 & 45 \\
     & Unif & 51 & 49 & 51 & 48 \\
     \bottomrule
    \end{tabular}
}
    
    \caption{\edite{ds-BLEU} (left) and $100\times$COMET (right) scores for \FTnllbII (FT) and \UNIFnllbII (Unif) trained on \tedII with target max source document length $M=2048$.  }

    \label{tab:res-nllb-ted-distill}
    \end{minipage}
\end{table*}



==> tabs/res-nllb-TED-unif-testsets-ds-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}

    \scalebox{0.72}{
        \begin{tabular}{rl|rrrr}
        \toprule
         &  & 2014 & 2015 & 2016 & 2017 \\
         \midrule
        \multirow[c]{2}{*}{sent} & FT & 44.2 \footnotesize{(0.99)} & 43.5 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.00)} & 41.4 \footnotesize{(1.00)} \\
         & Unif & 40.1 \footnotesize{(0.95)} & 40.4 \footnotesize{(0.97)} & 38.0 \footnotesize{(1.00)} & 38.1 \footnotesize{(0.99)} \\
         \midrule
        \multirow[c]{2}{*}{256} & FT & 43.2 \footnotesize{(0.98)} & 42.8 \footnotesize{(0.99)} & 39.7 \footnotesize{(1.00)} & 40.5 \footnotesize{(1.00)} \\
         & Unif & 42.8 \footnotesize{(0.98)} & 42.4 \footnotesize{(0.99)} & 39.5 \footnotesize{(1.00)} & 40.3 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{512} & FT & 42.9 \footnotesize{(0.98)} & 43.1 \footnotesize{(0.99)} & 39.2 \footnotesize{(1.00)} & 39.4 \footnotesize{(1.00)} \\
         & Unif & 43.4 \footnotesize{(0.98)} & 43.0 \footnotesize{(0.99)} & 39.8 \footnotesize{(1.00)} & 40.5 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{768} & FT & 43.5 \footnotesize{(0.98)} & 43.0 \footnotesize{(0.99)} & 39.4 \footnotesize{(1.00)} & 39.8 \footnotesize{(1.00)} \\
         & Unif & 44.0 \footnotesize{(0.98)} & 43.7 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.00)} & 40.9 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{1024} & FT & 42.6 \footnotesize{(0.96)} & 42.6 \footnotesize{(0.97)} & 39.2 \footnotesize{(1.00)} & 39.6 \footnotesize{(1.00)} \\
         & Unif & 42.6 \footnotesize{(0.96)} & 44.1 \footnotesize{(0.98)} & 39.6 \footnotesize{(1.00)} & 40.6 \footnotesize{(0.99)} \\
         \midrule
        \multirow[c]{2}{*}{1200} & FT & 38.3 \footnotesize{(0.88)} & 39.3 \footnotesize{(0.91)} & 36.3 \footnotesize{(0.92)} & 36.4 \footnotesize{(0.92)} \\
         & Unif & 39.5 \footnotesize{(0.89)} & 43.0 \footnotesize{(0.97)} & 38.0 \footnotesize{(0.95)} & 39.2 \footnotesize{(0.98)} \\
         \midrule
        \multirow[c]{2}{*}{1600} & FT & 31.5 \footnotesize{(0.77)} & 30.4 \footnotesize{(0.73)} & 30.9 \footnotesize{(0.83)} & 30.3 \footnotesize{(0.80)} \\
         & Unif & 31.5 \footnotesize{(0.72)} & 34.4 \footnotesize{(0.82)} & 34.2 \footnotesize{(0.88)} & 33.8 \footnotesize{(0.84)} \\
         \midrule
        \multirow[c]{2}{*}{2048} & FT & 27.4 \footnotesize{(0.69)} & 24.0 \footnotesize{(0.63)} & 26.7 \footnotesize{(0.75)} & 23.6 \footnotesize{(0.71)} \\
         & Unif & 30.2 \footnotesize{(0.68)} & 25.3 \footnotesize{(0.60)} & 31.5 \footnotesize{(0.79)} & 28.0 \footnotesize{(0.68)} \\
         \bottomrule
        \end{tabular}
    }

    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}

    \scalebox{0.72}{
    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT & 84 & 85 & 85 & 84 \\
     & Unif & 82 & 83 & 83 & 83 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT & 80 & 81 & 81 & 81 \\
     & Unif & 80 & 81 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT & 80 & 81 & 81 & 81 \\
     & Unif & 81 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT & 80 & 81 & 81 & 81 \\
     & Unif & 81 & 82 & 82 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT & 78 & 79 & 78 & 78 \\
     & Unif & 80 & 81 & 81 & 80 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT & 71 & 73 & 70 & 69 \\
     & Unif & 76 & 79 & 76 & 75 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT & 61 & 60 & 61 & 60 \\
     & Unif & 62 & 61 & 61 & 64 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT & 57 & 53 & 57 & 54 \\
     & Unif & 59 & 57 & 57 & 54 \\
     \bottomrule
    \end{tabular}

}
    
    \caption{\edite{ds-BLEU} (left) and $100\times$COMET (right) scores for \FTnllbI (FT) and \UNIFnllbI (Unif) trained on \tedI with target max source document length $M=2048$.  }
    \label{tab:res-nllb-ted-unif}
    \end{minipage}
\end{table*}



==> tabs/res-tower-TED-distill-testsets-ds-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}

        \scalebox{0.72}{

        \begin{tabular}{ll|rrrr}
        \toprule
         &  & 2014 & 2015 & 2016 & 2017 \\
         \midrule
        \multirow[c]{2}{*}{sent} & FT & 46.5 \footnotesize{(0.98)} & 45.1 \footnotesize{(0.99)} & 42.3 \footnotesize{(1.00)} & 41.0 \footnotesize{(1.00)} \\
         & Unif & 46.5 \footnotesize{(0.98)} & 45.0 \footnotesize{(0.99)} & 42.3 \footnotesize{(1.00)} & 41.1 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{256} & FT & 44.6 \footnotesize{(0.98)} & 45.1 \footnotesize{(0.99)} & 42.3 \footnotesize{(1.00)} & 41.9 \footnotesize{(1.00)} \\
         & Unif & 44.5 \footnotesize{(0.99)} & 45.1 \footnotesize{(0.99)} & 42.2 \footnotesize{(1.00)} & 41.8 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{512} & FT & 43.7 \footnotesize{(0.98)} & 45.0 \footnotesize{(1.00)} & 41.4 \footnotesize{(1.00)} & 41.6 \footnotesize{(1.00)} \\
         & Unif & 43.7 \footnotesize{(0.98)} & 44.8 \footnotesize{(1.00)} & 41.4 \footnotesize{(1.00)} & 41.4 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{768} & FT & 44.0 \footnotesize{(0.98)} & 44.2 \footnotesize{(0.99)} & 40.3 \footnotesize{(1.00)} & 40.7 \footnotesize{(1.00)} \\
         & Unif & 44.0 \footnotesize{(0.98)} & 44.2 \footnotesize{(0.99)} & 40.2 \footnotesize{(1.00)} & 40.7 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{1024} & FT & 42.7 \footnotesize{(0.98)} & 40.6 \footnotesize{(0.99)} & 38.9 \footnotesize{(1.00)} & 40.4 \footnotesize{(1.00)} \\
         & Unif & 42.2 \footnotesize{(0.97)} & 42.6 \footnotesize{(0.99)} & 39.4 \footnotesize{(1.00)} & 40.1 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{1200} & FT & 42.6 \footnotesize{(0.98)} & 43.0 \footnotesize{(0.99)} & 38.9 \footnotesize{(1.00)} & 40.8 \footnotesize{(1.00)} \\
         & Unif & 42.5 \footnotesize{(0.98)} & 42.7 \footnotesize{(0.99)} & 39.3 \footnotesize{(1.00)} & 40.6 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{1600} & FT & 42.0 \footnotesize{(0.97)} & 41.1 \footnotesize{(0.98)} & 37.0 \footnotesize{(1.00)} & 38.7 \footnotesize{(1.00)} \\
         & Unif & 42.0 \footnotesize{(0.97)} & 40.0 \footnotesize{(0.98)} & 37.5 \footnotesize{(1.00)} & 37.3 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{2048} & FT & 33.0 \footnotesize{(0.99)} & 32.5 \footnotesize{(0.99)} & 31.6 \footnotesize{(1.00)} & 29.2 \footnotesize{(0.97)} \\
         & Unif & 33.1 \footnotesize{(0.99)} & 33.7 \footnotesize{(0.99)} & 32.2 \footnotesize{(0.98)} & 26.5 \footnotesize{(0.97)} \\
         \bottomrule
        \end{tabular}
    
    }
    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}
    
    \scalebox{0.72}{
    \begin{tabular}{ll|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT & 85 & 86 & 85 & 85 \\
     & Unif & 85 & 86 & 85 & 85 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT & 83 & 84 & 83 & 83 \\
     & Unif & 83 & 84 & 83 & 83 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT & 82 & 84 & 83 & 82 \\
     & Unif & 82 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT & 82 & 83 & 83 & 82 \\
     & Unif & 82 & 83 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT & 81 & 81 & 82 & 81 \\
     & Unif & 81 & 82 & 83 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT & 78 & 82 & 81 & 81 \\
     & Unif & 78 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT & 80 & 79 & 79 & 80 \\
     & Unif & 79 & 78 & 79 & 78 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT & 68 & 69 & 68 & 64 \\
     & Unif & 69 & 70 & 70 & 62 \\
     \bottomrule
    \end{tabular}
    }
    \caption{\edite{ds-BLEU} (left) and $100\times$COMET (right) scores for \FTtowerII (FT) and \UNIFtowerII (Unif) trained on \tedII with target max source document length 2048 ($M = 4096$).}
    \label{tab:res-tower-ted-distill}
    \end{minipage}
\end{table*}



==> tabs/res-tower-TED-unif-testsets-ds-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}

       \scalebox{0.72}{
       \begin{tabular}{rl|rrrr}
       \toprule
         &  & 2014 & 2015 & 2016 & 2017 \\
         \midrule
        \multirow[c]{2}{*}{sent} & FT & 46.2 \footnotesize{(0.99)} & 45.1 \footnotesize{(0.99)} & 42.1 \footnotesize{(1.00)} & 40.8 \footnotesize{(1.00)} \\
         & Unif & 46.4 \footnotesize{(0.98)} & 45.1 \footnotesize{(0.99)} & 42.2 \footnotesize{(1.00)} & 40.9 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{256} & FT & 46.3 \footnotesize{(0.98)} & 45.1 \footnotesize{(0.99)} & 42.3 \footnotesize{(1.00)} & 41.8 \footnotesize{(1.00)} \\
         & Unif & 44.5 \footnotesize{(0.98)} & 45.2 \footnotesize{(0.99)} & 42.3 \footnotesize{(1.00)} & 41.9 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{512} & FT & 44.4 \footnotesize{(0.98)} & 44.9 \footnotesize{(0.99)} & 41.2 \footnotesize{(1.00)} & 41.6 \footnotesize{(1.00)} \\
         & Unif & 43.0 \footnotesize{(0.98)} & 45.0 \footnotesize{(0.99)} & 41.4 \footnotesize{(1.00)} & 41.6 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{768} & FT & 44.1 \footnotesize{(0.98)} & 44.6 \footnotesize{(0.99)} & 41.1 \footnotesize{(1.00)} & 40.8 \footnotesize{(1.00)} \\
         & Unif & 43.2 \footnotesize{(0.99)} & 44.5 \footnotesize{(0.99)} & 41.4 \footnotesize{(1.00)} & 41.0 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{1024} & FT & 43.9 \footnotesize{(0.97)} & 41.6 \footnotesize{(0.99)} & 39.6 \footnotesize{(1.00)} & 39.7 \footnotesize{(1.00)} \\
         & Unif & 42.7 \footnotesize{(0.98)} & 43.8 \footnotesize{(0.99)} & 39.7 \footnotesize{(1.00)} & 39.6 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{1200} & FT & 43.2 \footnotesize{(0.97)} & 42.9 \footnotesize{(0.99)} & 39.5 \footnotesize{(1.00)} & 40.8 \footnotesize{(1.00)} \\
         & Unif & 43.2 \footnotesize{(0.98)} & 43.1 \footnotesize{(0.99)} & 38.2 \footnotesize{(1.00)} & 40.9 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{1600} & FT & 41.6 \footnotesize{(0.95)} & 40.5 \footnotesize{(0.97)} & 37.6 \footnotesize{(1.00)} & 39.8 \footnotesize{(0.99)} \\
         & Unif & 41.1 \footnotesize{(0.97)} & 41.6 \footnotesize{(0.98)} & 36.5 \footnotesize{(1.00)} & 38.0 \footnotesize{(1.00)} \\
         \midrule
        \multirow[c]{2}{*}{2048} & FT & 34.4 \footnotesize{(0.96)} & 35.3 \footnotesize{(0.97)} & 31.2 \footnotesize{(0.99)} & 28.2 \footnotesize{(0.96)} \\
         & Unif & 34.6 \footnotesize{(0.97)} & 35.5 \footnotesize{(0.98)} & 30.2 \footnotesize{(1.00)} & 30.9 \footnotesize{(0.97)} \\
         \bottomrule
        \end{tabular}
    }

    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}

        \scalebox{0.72}{
    
    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT & 85 & 86 & 85 & 85 \\
     & Unif & 85 & 86 & 85 & 85 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT & 83 & 84 & 83 & 83 \\
     & Unif & 83 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT & 82 & 84 & 83 & 82 \\
     & Unif & 82 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT & 82 & 83 & 83 & 82 \\
     & Unif & 82 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT & 81 & 81 & 83 & 81 \\
     & Unif & 81 & 83 & 83 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT & 80 & 82 & 81 & 81 \\
     & Unif & 80 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT & 79 & 79 & 80 & 80 \\
     & Unif & 80 & 80 & 78 & 79 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT & 68 & 72 & 69 & 64 \\
     & Unif & 70 & 72 & 69 & 67 \\
     \bottomrule
    \end{tabular}
    }
    
    \caption{\edite{ds-BLEU} (left) and $100\times$COMET (right) for \FTtowerI (FT) and \UNIFtowerI (Unif) trained on \tedI with target max source document length 2048 ($M = 4096$).}
    \label{tab:res-tower-ted-unif}
    \end{minipage}
\end{table*}



==> tabs/stat-no-repetition-nllb-tower.tex <==



\begin{table}
  \centering
    \scalebox{0.7}{

    \begin{tabular}{lrrrrlll}
    \toprule
     & 256 & 512 & 768 & 1024 & 1200 & 1600 & 2048 \\
     \midrule
    NLLB & 0.96 & 0.65 & 0.51 & 0.34 & - & - & - \\
    FT-D1 & 0.99 & 0.97 & 0.92 & 0.91 & 0.87 & 0.74 & 0.56 \\
    % Unif-r7-D1 & 0.99 & 0.95 & 0.92 & 0.75 & 0.67 & 0.59 & 0.54 \\
    Unif-D1 & 0.99 & 0.97 & 0.93 & 0.90 & 0.80 & 0.66 & 0.68 \\
    FT-D2 & 0.99 & 0.97 & 0.89 & 0.69 & 0.60 & 0.43 & 0.31 \\
    % Unif-r7-D2 & 0.98 & 0.95 & 0.79 & 0.78 & 0.70 & 0.68 & 0.57 \\
    Unif-D2 & 0.99 & 0.96 & 0.84 & 0.80 & 0.73 & 0.75 & 0.64 \\
    \bottomrule
    \end{tabular}
    }  

    \medskip
    
    \scalebox{0.7}{
    \begin{tabular}{lrrrrrrr}
    \toprule
     & 256 & 512 & 768 & 1024 & 1200 & 1600 & 2048 \\
     \midrule
    Tower & 0.99 & 0.95 & 0.82 & 0.75 & 0.70 & 0.64 & 0.45 \\
    FT-D1 & 0.99 & 0.95 & 0.90 & 0.85 & 0.87 & 0.77 & 0.41 \\
    % Unif-r7-D1 & 0.99 & 0.95 & 0.91 & 0.85 & 0.89 & 0.76 & 0.40 \\
    Unif-D1 & 0.98 & 0.95 & 0.91 & 0.85 & 0.84 & 0.72 & 0.39 \\
    FT-D2 & 0.98 & 0.95 & 0.90 & 0.85 & 0.81 & 0.74 & 0.38 \\
    % Unif-r7-D2 & 0.98 & 0.93 & 0.91 & 0.85 & 0.80 & 0.66 & 0.39 \\
    Unif-D2 & 0.98 & 0.93 & 0.90 & 0.84 & 0.80 & 0.72 & 0.36 \\
    \bottomrule
    \end{tabular}

    }  
    \caption{Percentage of pseudo-documents among IWSLT \testset{tst2014-2017} in which no $10$gram repetition is detected from the translation given by \model{NLLB}-based (top) and \model{TowerBase}-based models (bottom).}
  \label{tab:stat-no-repeat}
\end{table}

==> tabs/ttest-begin-id-eval-position-nllb-tower.tex <==
\begin{table}
  \centering
    \scalebox{0.68}{
    % \setlength{\tabcolsep}{5pt}
    \begin{tabular}{lrrrrr}
    \toprule
     & \model{NLLB} & FT-U & Unif-U & FT-G & Unif-G \\
     \midrule
    $p_0$-$p_1$ & 12.7 \footnotesize{(0.00)} & - & - & 1.6 \footnotesize{(0.00)} & 3.0 \footnotesize{(0.00)} \\
    $p_0$-$p_1$ & 7.2 \footnotesize{(0.00)} & - & - & 1.9 \footnotesize{(0.00)} & 2.4 \footnotesize{(0.00)} \\
    $p_2$-$p_3$ & 2.9 \footnotesize{(0.00)} & 1.0 \footnotesize{(0.00)} & -1.3 \footnotesize{(0.00)} & 2.4 \footnotesize{(0.00)} & - \\
    $p_3$-$p_4$ & 7.2 \footnotesize{(0.00)} & 5.5 \footnotesize{(0.00)} & 4.6 \footnotesize{(0.00)} & 26.1 \footnotesize{(0.00)} & 10.7 \footnotesize{(0.00)} \\
    $p_4$-$p_5$ & - & 3.9 \footnotesize{(0.00)} & - & 8.3 \footnotesize{(0.00)} & 4.7 \footnotesize{(0.00)} \\
    $p_5$-$p_6$ & 3.3 \footnotesize{(0.00)} & 31.6 \footnotesize{(0.00)} & 27.1 \footnotesize{(0.00)} & 6.1 \footnotesize{(0.00)} & 15.4 \footnotesize{(0.00)} \\
    \bottomrule
    \end{tabular}
    }  

    \medskip
    \setlength{\tabcolsep}{4pt}
    \scalebox{0.68}{
    
    \begin{tabular}{lrrrrr}
    \toprule
     & \model{Tower} & FT-U & Unif-U & FT-G & Unif-G \\
     \midrule
    $p_0$-$p_1$ & 1.2 (0.02) & - & - & - & - \\
    $p_1$-$p_2$  & - & - & - & 0.6 (0.01) & 0.6 (0.01) \\
    $p_2$-$p_3$ & - & - & - & - & - \\
    $p_3$-$p_4$ & 4.9 (0.00) & 1.1 (0.00) & 0.6 (0.04) & 1.1 (0.00) & 1.3 (0.00) \\
    $p_4$-$p_5$ & 1.7 (0.02) & 1.4 (0.00) & 2.1 (0.00) & 2.0 (0.00) & 1.8 (0.00) \\
    $p_5$-$p_6$ & 26.3 (0.00) & 24.5 (0.00) & 26.0 (0.00) & 27.1 (0.00) & 26.4 (0.00) \\
    \bottomrule
    \end{tabular}
    } 

    \caption{Average difference (and p-values) of $100\times$COMET-score evaluated on $794$ sentence pairs, translated at different positions by \model{NLLB}-based systems (top) and \model{TowerBase}-based systems (bottom). \rebuttal{- for p-values $> 0.05$.}  
    }
    % Each sentence $s_j$ has been translated in seven different positions $\{p_0^j, \dots, p_6^j\}$ across our 28 test sets. The average values of $\{p_0^j, \dots, p_6^j\}$ for all these sentences are $\{p_0, \dots, p_6\} = [66, 173, 262, 335, 585, 779, 1477]$ respectively.
  \label{tab:ttest-position-nllb-tower}
\end{table}

==> tabs/ttest-by-block-all.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.48\textwidth}
    \scalebox{0.65}{
    \begin{tabular}{rrrrrr}
    \toprule
     & \multicolumn{1}{c}{\model{NLLB}} & \multicolumn{1}{c}{FT-U} & \multicolumn{1}{c}{Unif-U} & \multicolumn{1}{c}{FT-G} & \multicolumn{1}{c}{Unif-G} \\
     \midrule
    sent-256 & 9.2 \footnotesize{(0.00)} & 0.8 \footnotesize{(0.00)} & -2.1 \footnotesize{(0.00)} & 0.4 \footnotesize{(0.03)} & -0.7 \footnotesize{(0.00)} \\
    256-512 & 19.1 \footnotesize{(0.00)} & - & -0.4 \footnotesize{(0.03)} & - & - \\
    512-768 & 6.9 \footnotesize{(0.00)} & - & -0.6 \footnotesize{(0.00)} & 5.9 \footnotesize{(0.00)} & 2.5 \footnotesize{(0.00)} \\
    768-1024 & - & 0.5 \footnotesize{(0.01)} & - & 7.2 \footnotesize{(0.00)} & 3.0 \footnotesize{(0.00)} \\
    1024-1200 & 2.2 \footnotesize{(0.00)} & 3.5 \footnotesize{(0.00)} & 1.9 \footnotesize{(0.00)} & 4.0 \footnotesize{(0.00)} & 3.3 \footnotesize{(0.00)} \\
    1200-1600 & - & 6.8 \footnotesize{(0.00)} & 6.5 \footnotesize{(0.00)} & 5.8 \footnotesize{(0.00)} & 5.5 \footnotesize{(0.00)} \\
    1600-2048 & 1.9 \footnotesize{(0.00)} & 5.2 \footnotesize{(0.00)} & 4.5 \footnotesize{(0.00)} & 4.2 \footnotesize{(0.00)} & 5.7 \footnotesize{(0.00)} \\
    % \bottomrule
    % \end{tabular}
    % }  
    % \medskip
    
    % \scalebox{0.68}{
    % \begin{tabular}{lrrrrr}
    % \toprule
    %  & \multicolumn{1}{c}{NLLB} & \multicolumn{1}{c}{FT-D1} & \multicolumn{1}{c}{Unif-D1} & \multicolumn{1}{c}{FT-D2} & \multicolumn{1}{c}{Unif-D2} \\
     \midrule
    sent-256 & 16.7 \footnotesize{(0.00)} & 3.5 \footnotesize{(0.00)} & 1.7 \footnotesize{(0.00)} & 2.7 \footnotesize{(0.00)} & 2.1 \footnotesize{(0.00)} \\
    256-512 & 20.7 \footnotesize{(0.00)} & - & -0.4 \footnotesize{(0.03)} & 0.6 \footnotesize{(0.00)} & - \\
    512-768 & 5.6 \footnotesize{(0.00)} & - & - & 11.6 \footnotesize{(0.00)} & 7.2 \footnotesize{(0.00)} \\
    768-1024 & 5.2 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} & 0.8 \footnotesize{(0.04)} & 10.4 \footnotesize{(0.00)} & 7.6 \footnotesize{(0.00)} \\
    1024-1200 & - & 7.4 \footnotesize{(0.00)} & 4.3 \footnotesize{(0.00)} & 3.8 \footnotesize{(0.00)} & 4.7 \footnotesize{(0.00)} \\
    1200-1600 & 6.1 \footnotesize{(0.0)} & 9.6 \footnotesize{(0.00)} & 13.4 \footnotesize{(0.00)} & 5.4 \footnotesize{(0.00)} & 5.5 \footnotesize{(0.00)} \\
    1600-2048 & - & 5.1 \footnotesize{(0.00)} & 5.0 \footnotesize{(0.00)} & 3.9 \footnotesize{(0.00)} & 5.6 \footnotesize{(0.00)} \\
    \bottomrule
    \end{tabular}
    }   
    % \caption{Average differences (and p-values) evaluated on \textbf{ds-BLEU} for full TED talks (top) and on $100\times$\textbf{COMET} for realigned sentences (bottom), for \model{NLLB} models. Only p-values $< 0.05$ are reported. D1 and D2 denote \tedI and \tedII respectively. }
    % \label{tab:ttest-by-block-nllb}
    \end{minipage}%
    \hspace{0.02\textwidth} % Space between tables
    \begin{minipage}{0.48\textwidth}
    \scalebox{0.65}{
    \begin{tabular}{rrrrrr}
    \toprule
     & \model{Tower} & FT-U & Unif-U & FT-G & Unif-G \\
     \midrule
    sent-256 & - & - & - & - & - \\
    256-512 & - & 0.9 \footnotesize{(0.02)} & 0.8 \footnotesize{(0.05)} & 0.6 \footnotesize{(0.00)} & 0.6 \footnotesize{(0.00)} \\
    512-768 & - & - & - & 0.6 \footnotesize{(0.04)} & - \\
    768-1024 & 3.4 \footnotesize{(0.00)} & - & 1.0 \footnotesize{(0.05)} & 1.7 \footnotesize{(0.01)} & 1.2 \footnotesize{(0.01)} \\
    1024-1200 & - & - & - & - & - \\
    1200-1600 & 4.7 \footnotesize{(0.00)} & 1.7 \footnotesize{(0.01)} & 2.1 \footnotesize{(0.01)} & 1.6 \footnotesize{(0.02)} & 2.0 \footnotesize{(0.01)} \\
    1600-2048 & 5.9 \footnotesize{(0.00)} & 7.5 \footnotesize{(0.00)} & 6.5 \footnotesize{(0.00)} & 8.1 \footnotesize{(0.00)} & 7.8 \footnotesize{(0.00)} \\
    % \bottomrule
    % \end{tabular}
    % }
    % \medskip

    % \scalebox{0.68}{
    % \begin{tabular}{lrrrrr}
    % \toprule
    %  & Tower & FT-D1 & Unif-D1 & FT-D2 & Unif-D2 \\
     \midrule
    sent-256 & 3.9 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} & 2.4 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} & 2.3 \footnotesize{(0.00)} \\
    256-512 & - & 0.4 \footnotesize{(0.02)} & - & 0.2 \footnotesize{(0.03)} & 0.3 \footnotesize{(0.02)} \\
    512-768 & - & - & - & 0.3 \footnotesize{(0.00)} & - \\
    768-1024 & 2.9 \footnotesize{(0.00)} & 1.0 \footnotesize{(0.04)} & 0.5 \footnotesize{(0.00)} & 1.1 \footnotesize{(0.03)} & 0.8 \footnotesize{(0.00)} \\
    1024-1200 & - & - & 1.0 \footnotesize{(0.03)} & - & - \\
    1200-1600 & 6.2 \footnotesize{(0.00)} & 1.7 \footnotesize{(0.00)} & 1.8 \footnotesize{(0.02)} & - & 1.9 \footnotesize{(0.01)} \\
    1600-2048 & 8.7 \footnotesize{(0.00)} & 10.0 \footnotesize{(0.00)} & 8.9 \footnotesize{(0.00)} & 11.0 \footnotesize{(0.00)} & 10.2 \footnotesize{(0.00)} \\
    \bottomrule
    \end{tabular}
    }
    \caption{Average differences (and p-values) evaluated on \textbf{ds-BLEU} (top) of full TED talks and on $100\times$\textbf{COMET} (bottom) of realigned parallel sentences, for \model{NLLB} (left) and \model{TowerBase} (right) models. - for p-values $> 0.05$. U and G respectively denote \tedI and \tedII.  }
    \end{minipage}
    \label{tab:ttest-by-block}
    % \rebuttal{A positive value means that shorter segments yield higher scores than longer ones.}
\end{table*}
% `nan' marks no translated test sets.


    
    %     (e.g.\ $9.2$ in line ``sent-256'' in Table~\ref{tab:ttest-by-block}) means that shorter segments (here: sentences) yield higher scores than longer ones ($256$ tokens).}
    % A positive value (e.g.\ $9.2$ in line ``sent-256'') means that the translation of shorter segments (here: sentences) yield better scores than that of longer ones ($256$ tokens).
    
% \footnote{ \rebuttal{In Table~\Cref{tab:ttest-by-block,tab:ttest-compare-system-nllb,tab:ttest-compare-system-base-ft,tab:ttest-compare-system-tower}, a positive value indicates that in the paired comparison, the translation of the former one (e.g.\ sentences in ``sent-256'' for \model{NLLB} in Table\ref{tab:ttest-by-block}, FT in ``FT vs Unif'' for sentences) yield better scores than that of the latter one. } }

% \rebuttal{A positive value means that in the paired comparison, the translation of the former one (e.g.\ sentences in ``sent-256'' for \model{NLLB}) yield better scores than the latter one. Similarly for \Cref{tab:ttest-compare-system-nllb,tab:ttest-compare-system-tower}.} 


==> tabs/ttest-compare-system-nllb.tex <==


\begin{table}
  \centering
  \setlength{\tabcolsep}{4pt}
    \scalebox{0.68}{
    \begin{tabular}{r|cc|cc}
    \toprule
     & \tedI & \tedII & FT & Unif \\
     % & FT vs Unif & FT vs Unif & \tedI vs \tedII & \tedI vs \tedII \\
     & FT vs Unif & FT vs Unif &  U vs G & U vs G \\
     % & FT -  Unif & FT -  Unif & U -  G & U -  G \\
     
     \midrule
    sent & 3.3 \footnotesize{(0.00)} & 1.2 \footnotesize{(0.00)} & - & -2.1 \footnotesize{(0.00)} \\
    256 & - & - & - & -0.6 \footnotesize{(0.01)} \\
        512 & -0.5 \footnotesize{(0.01)} & - & -0.7 \footnotesize{(0.00)} & \highlight{-0.4 \footnotesize{(0.01)}} \\
    768 & -0.8 \footnotesize{(0.00)} & -3.7 \footnotesize{(0.00)} & 5.5 \footnotesize{(0.00)} & 2.6 \footnotesize{(0.00)} \\
    1024 & - & -7.8 \footnotesize{(0.00)} & 12.2 \footnotesize{(0.00)} & 5.1 \footnotesize{(0.00)} \\
    1200 & -2.3 \footnotesize{(0.00)} & -8.5 \footnotesize{(0.00)} & 12.7 \footnotesize{(0.00)} & 6.5 \footnotesize{(0.00)} \\
    1600 & \highlight{-2.6 \footnotesize{(0.01)}} & -8.8 \footnotesize{(0.00)} & 11.8 \footnotesize{(0.00)} & 5.6 \footnotesize{(0.00)} \\
    2048 & \highlight{-3.3 \footnotesize{(0.00)}} & -7.3 \footnotesize{(0.00)} & 10.7 \footnotesize{(0.00)} & 6.8 \footnotesize{(0.00)} \\ 
    % \midrule
    % \end{tabular}
    % }  

  %   \medskip

  % \setlength{\tabcolsep}{4pt}
  %   \scalebox{0.68}{
  %   \begin{tabular}{l*{2}{|*{2}{c}}}
  %   \toprule
  %    & D1 & D2 & FT & Unif \\
  %    & FT vs Unif & FT vs Unif & D1 vs D2 & D1 vs D2 \\
     \midrule
    sent & 1.9 \footnotesize{(0.00)} & 0.9 \footnotesize{(0.00)} & - & -0.9 \footnotesize{(0.00)} \\
    256 & - & \highlight{0.4 \footnotesize{(0.00)}} & \highlight{-0.8 \footnotesize{(0.00)}} & -0.5 \footnotesize{(0.01)} \\
    512 & -0.6 \footnotesize{(0.02)} & - & -0.4 \footnotesize{(0.03)} & - \\
    768 & -0.7 \footnotesize{(0.00)} & -4.7 \footnotesize{(0.00)} & 11.2 \footnotesize{(0.00)} & 7.2 \footnotesize{(0.00)} \\
    1024 & \highlight{-2.2 \footnotesize{(0.00)}} & -7.5 \footnotesize{(0.00)} & 19.3 \footnotesize{(0.00)} & 14.0 \footnotesize{(0.00)} \\
    1200 & -5.3 \footnotesize{(0.00)} & -6.5 \footnotesize{(0.00)} & 15.7 \footnotesize{(0.00)} & 14.5 \footnotesize{(0.00)} \\
    1600 & - & -6.4 \footnotesize{(0.00)} & 11.5 \footnotesize{(0.00)} & 6.6 \footnotesize{(0.00)} \\
    2048 & - & -4.7 \footnotesize{(0.00)} & 10.4 \footnotesize{(0.00)} & 7.2 \footnotesize{(0.00)} \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Average difference (and p-values) in \textbf{ds-BLEU} (top) evaluated on full TED talks and $100\times$\textbf{COMET} (bottom) evaluated on realigned sentences for \model{NLLB}. \rebuttal{- for p-values $> 0.05$.}
    Left:  scores without and with \posUnif; right: scores of fine-tuning on \tedI (U) or \tedII(G).
    \rebuttal{Bold text marks differences significant for one metric but not for another.}
    } 
  \label{tab:ttest-compare-system-nllb}
\end{table}
\done{time permitting, make columns with even length}
% \rebuttal{difference between}

==> tabs/ttest-compare-system-tower-no-significative.tex <==


\begin{table}
  \centering
  \setlength{\tabcolsep}{4pt}
    \scalebox{0.8}{
    \begin{tabular}{r|cc|cc}
    \toprule
     & \tedI & \tedII & FT & Unif \\
     & FT vs Unif & FT vs Unif & U vs G & U vs G \\
     \midrule
    sent & -0.1 \footnotesize{(0.20)} & -0.0 \footnotesize{(0.60)} & -0.1 \footnotesize{\textbf{(0.05)}} & -0.1 \footnotesize{(0.19)} \\
    256 & 0.5 \footnotesize{(0.32)} & 0.1 \footnotesize{(0.22)} & 0.5 \footnotesize{(0.32)} & 0.1 \footnotesize{(0.21)} \\
    512 & 0.3 \footnotesize{(0.55)} & 0.1 \footnotesize{(0.08)} & 0.1 \footnotesize{(0.87)} & -0.1 \footnotesize{(0.82)} \\
    768 & 0.2 \footnotesize{(0.46)} & 0.0 \footnotesize{(0.84)} & 0.3 \footnotesize{(0.11)} & 0.2 \footnotesize{(0.65)} \\
    1024 & -0.2 \footnotesize{(0.82)} & -0.4 \footnotesize{(0.44)} & 0.6 \footnotesize{(0.29)} & 0.4 \footnotesize{(0.34)} \\
    1200 & 0.2 \footnotesize{(0.44)} & 0.0 \footnotesize{(0.70)} & 0.3 \footnotesize{(0.24)} & 0.1 \footnotesize{(0.71)} \\
    1600 & 0.6 \footnotesize{(0.45)} & 0.4 \footnotesize{(0.58)} & 0.1 \footnotesize{(0.84)} & 0.0 \footnotesize{(1.00)} \\
    2048 & -0.5 \footnotesize{(0.61)} & 0.2 \footnotesize{(0.84)} & 0.7 \footnotesize{(0.46)} & 1.3 \footnotesize{(0.13)} \\    
    \bottomrule
    \end{tabular}
}
    \medskip

  \setlength{\tabcolsep}{4pt}
    \scalebox{0.8}{
    \begin{tabular}{r|cc|cc}
    \toprule
     & \tedI & \tedII & FT & Unif \\
     & FT vs Unif & FT vs Unif & U vs G & U vs G \\
     \midrule
    sent & -0.0 \footnotesize{(0.52)} & 0.0 \footnotesize{(0.38)} & -0.0 \footnotesize{(0.95)} & 0.0 \footnotesize{(0.24)} \\
    256 & 0.0 \footnotesize{(0.60)} & 0.0 \footnotesize{(0.73)} & -0.0 \footnotesize{(0.63)} & -0.1 \footnotesize{(0.46)} \\
    512 & -0.1 \footnotesize{(0.15)} & 0.1 \footnotesize{(0.16)} & -0.2 \footnotesize{(0.09)} & 0.0 \footnotesize{(0.76)} \\
    768 & -0.1 \footnotesize{(0.29)} & -0.1 \footnotesize{(0.34)} & 0.0 \footnotesize{(0.87)} & 0.0 \footnotesize{(0.69)} \\
    1024 & -0.6 \footnotesize{(0.22)} & -0.3 \footnotesize{(0.46)} & 0.1 \footnotesize{(0.45)} & 0.3 \footnotesize{(0.10)} \\
    1200 & 0.1 \footnotesize{(0.69)} & 0.1 \footnotesize{(0.50)} & 0.1 \footnotesize{(0.61)} & 0.0 \footnotesize{(0.93)} \\
    1600 & 0.2 \footnotesize{(0.69)} & 0.6 \footnotesize{(0.37)} & -0.2 \footnotesize{(0.62)} & 0.2 \footnotesize{(0.73)} \\
    2048 & -0.9 \footnotesize{(0.40)} & -0.2 \footnotesize{(0.84)} & 0.9 \footnotesize{(0.50)} & 1.5 \footnotesize{(0.10)} \\
    \bottomrule
    \end{tabular}

    }
    
    \caption{Average difference (and p-value of paired t-test) of ds-BLEU (top) evaluated on concatenated full TED talk and $100\times$COMET (bottom) evaluated on realigned sentences, between \model{FT-TowerBase} (FT) and \model{Unif-TowerBase} (Unif), trained on \tedI (U) or \tedII(G).
    \rebuttal{A positive value indicates that in the paired comparison, the translation of the former one results in higher scores than the latter one.}
    }  
  \label{tab:ttest-compare-system-tower}
\end{table}


==> tabs/ttest-nllb-by-block.tex <==
\begin{table}
  \centering
    \scalebox{0.68}{
    \begin{tabular}{lrrrrr}
    \toprule
     & \multicolumn{1}{c}{NLLB} & \multicolumn{1}{c}{FT-D1} & \multicolumn{1}{c}{Unif-D1} & \multicolumn{1}{c}{FT-D2} & \multicolumn{1}{c}{Unif-D2} \\
     \midrule
    sent-256 & 9.2 \footnotesize{(0.0)} & 0.8 \footnotesize{(0.0)} & -2.1 \footnotesize{(0.0)} & 0.4 \footnotesize{(0.03)} & -0.7 \footnotesize{(0.0)} \\
    256-512 & 19.1 \footnotesize{(0.0)} & - & -0.4 \footnotesize{(0.03)} & - & - \\
    512-768 & 6.9 \footnotesize{(0.0)} & - & -0.6 \footnotesize{(0.0)} & 5.9 \footnotesize{(0.0)} & 2.5 \footnotesize{(0.0)} \\
    768-1024 & - & 0.5 \footnotesize{(0.01)} & - & 7.2 \footnotesize{(0.0)} & 3.0 \footnotesize{(0.0)} \\
    1024-1200 & nan & 3.5 \footnotesize{(0.0)} & 1.9 \footnotesize{(0.0)} & 4.0 \footnotesize{(0.0)} & 3.3 \footnotesize{(0.0)} \\
    1200-1600 & nan & 6.8 \footnotesize{(0.0)} & 6.5 \footnotesize{(0.0)} & 5.8 \footnotesize{(0.0)} & 5.5 \footnotesize{(0.0)} \\
    1600-2048 & nan & 5.2 \footnotesize{(0.0)} & 4.5 \footnotesize{(0.0)} & 4.2 \footnotesize{(0.0)} & 5.7 \footnotesize{(0.0)} \\
    \bottomrule
    \end{tabular}

    }  
    \medskip
    
    \scalebox{0.68}{
    \begin{tabular}{lrrrrr}
    \toprule
     & \multicolumn{1}{c}{NLLB} & \multicolumn{1}{c}{FT-D1} & \multicolumn{1}{c}{Unif-D1} & \multicolumn{1}{c}{FT-D2} & \multicolumn{1}{c}{Unif-D2} \\
     \midrule

    sent-256 & 16.7 \footnotesize{(0.0)} & 3.5 \footnotesize{(0.0)} & 1.7 \footnotesize{(0.0)} & 2.7 \footnotesize{(0.0)} & 2.1 \footnotesize{(0.0)} \\
    256-512 & 20.7 \footnotesize{(0.0)} & - & -0.4 \footnotesize{(0.03)} & 0.6 \footnotesize{(0.0)} & - \\
    512-768 & 5.6 \footnotesize{(0.0)} & - & - & 11.6 \footnotesize{(0.0)} & 7.2 \footnotesize{(0.0)} \\
    768-1024 & 5.2 \footnotesize{(0.0)} & 2.3 \footnotesize{(0.0)} & 0.8 \footnotesize{(0.04)} & 10.4 \footnotesize{(0.0)} & 7.6 \footnotesize{(0.0)} \\
    1024-1200 & nan & 7.4 \footnotesize{(0.0)} & 4.3 \footnotesize{(0.0)} & 3.8 \footnotesize{(0.0)} & 4.7 \footnotesize{(0.0)} \\
    1200-1600 & nan & 9.6 \footnotesize{(0.0)} & 13.4 \footnotesize{(0.0)} & 5.4 \footnotesize{(0.0)} & 5.5 \footnotesize{(0.0)} \\
    1600-2048 & nan & 5.1 \footnotesize{(0.0)} & 5.0 \footnotesize{(0.0)} & 3.9 \footnotesize{(0.0)} & 5.6 \footnotesize{(0.0)} \\
    \bottomrule
    \end{tabular}
    }   
    \caption{Average differences (and p-values) evaluated on \textbf{ds-BLEU} for full TED talks (top) and on $100\times$\textbf{COMET} for realigned sentences (bottom), for \model{NLLB} models. Only p-values $< 0.05$ are reported. D1 and D2 denote \tedI and \tedII respectively. }
  \label{tab:ttest-by-block-nllb}
\end{table}



==> tabs/ttest-tower-by-block.tex <==
\begin{table}
  \centering
    \scalebox{0.7}{
    \begin{tabular}{llllll}
    \toprule
     & Tower & FT-D1 & Unif-D1 & FT-D2 & Unif-D2 \\
     \midrule
    sent-256 & - & - & - & - & - \\
    256-512 & - & 0.9 \footnotesize{(0.02)} & 0.8 \footnotesize{(0.05)} & 0.6 \footnotesize{(0.0)} & 0.6 \footnotesize{(0.0)} \\
    512-768 & - & - & - & 0.6 \footnotesize{(0.04)} & - \\
    768-1024 & 3.4 \footnotesize{(0.0)} & - & 1.0 \footnotesize{(0.05)} & 1.7 \footnotesize{(0.01)} & 1.2 \footnotesize{(0.01)} \\
    1024-1200 & - & - & - & - & - \\
    1200-1600 & 4.7 \footnotesize{(0.0)} & 1.7 \footnotesize{(0.01)} & 2.1 \footnotesize{(0.01)} & 1.6 \footnotesize{(0.02)} & 2.0 \footnotesize{(0.01)} \\
    1600-2048 & 5.9 \footnotesize{(0.0)} & 7.5 \footnotesize{(0.0)} & 6.5 \footnotesize{(0.0)} & 8.1 \footnotesize{(0.0)} & 7.8 \footnotesize{(0.0)} \\
    \bottomrule
    \end{tabular}
    }
    \medskip

    \scalebox{0.7}{
    \begin{tabular}{lrrrrr}
    \toprule
     & Tower & FT-D1 & Unif-D1 & FT-D2 & Unif-D2 \\
     \midrule
    sent-256 & 3.9 \footnotesize{(0.0)} & 2.3 \footnotesize{(0.0)} & 2.4 \footnotesize{(0.0)} & 2.3 \footnotesize{(0.0)} & 2.3 \footnotesize{(0.0)} \\
    256-512 & - & 0.4 \footnotesize{(0.02)} & - & 0.2 \footnotesize{(0.03)} & 0.3 \footnotesize{(0.02)} \\
    512-768 & - & - & - & 0.3 \footnotesize{(0.0)} & - \\
    768-1024 & 2.9 \footnotesize{(0.0)} & 1.0 \footnotesize{(0.04)} & 0.5 \footnotesize{(0.0)} & 1.1 \footnotesize{(0.03)} & 0.8 \footnotesize{(0.0)} \\
    1024-1200 & - & - & 1.0 \footnotesize{(0.03)} & - & - \\
    1200-1600 & 6.2 \footnotesize{(0.0)} & 1.7 \footnotesize{(0.0)} & 1.8 \footnotesize{(0.02)} & - & 1.9 \footnotesize{(0.01)} \\
    1600-2048 & 8.7 \footnotesize{(0.0)} & 10.0 \footnotesize{(0.0)} & 8.9 \footnotesize{(0.0)} & 11.0 \footnotesize{(0.0)} & 10.2 \footnotesize{(0.0)} \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Average differences (and p-values) evaluated on \textbf{ds-BLEU} (top) of full TED talks and on $100\times$\textbf{COMET} (bottom) of realigned parallel sentences, for \model{TowerBase} models. - for p-values $> 0.05$. D1 and D2 respectively denote \tedI and \tedII.  }
  \label{tab:ttest-by-block-tower}
\end{table}


==> tabs/vanilla-bleu/res-backbone-models-vanilla-bleu.tex <==


\begin{table}
  \centering
    \scalebox{0.76}{
    \begin{tabular}{lr|rrrr}
    \toprule
    & $l_{max}$ & 2014 & 2015 & 2016 & 2017 \\
    \midrule
    \parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\model{NLLB}}}} &
    sent & 42.8 \footnotesize{(0.98)} & 41.2 \footnotesize{(1.00)} & 39.7 \footnotesize{(1.00)} & 39.1 \footnotesize{(1.00)} \\
    & 256 & 31.1 \footnotesize{(0.82)} & 31.6 \footnotesize{(0.84)} & 30.4 \footnotesize{(0.86)} & 29.5 \footnotesize{(0.86)} \\
    & 512 & 12.3 \footnotesize{(0.47)} & 12.7 \footnotesize{(0.60)} & 11.2 \footnotesize{(0.53)} & 10.8 \footnotesize{(0.49)} \\
    & 768 & 6.1 \footnotesize{(0.28)} & 6.7 \footnotesize{(0.34)} & 7.0 \footnotesize{(0.52)} & 5.2 \footnotesize{(0.26)} \\
    & 1024 & 5.7 \footnotesize{(0.66)} & 5.3 \footnotesize{(0.54)} & 4.6 \footnotesize{(0.59)} & 4.4 \footnotesize{(0.55)} \\
%     \bottomrule
%     \end{tabular}
% }
% % \caption{Vanilla-BLEU evaluated on \model{NLLB200-distilled-600M} }
% %   \label{tab:res-base-bleu-nllb}
% % \end{table}
% % \begin{table}
% %   \centering
%     \smallskip
    
%     \scalebox{0.76}{
%     % prompt English $SRC\nFrench:
%     \begin{tabular}{l|rrrr}
%     \toprule
%      $l_{max}$ & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \parbox[t]{3mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\model{TowerBase}}}} &
    sent & 41.3 \footnotesize{(1.00)} & 39.8 \footnotesize{(1.00)} & 37.7 \footnotesize{(1.00)} & 35.0 \footnotesize{(1.00)} \\
    & 256 & 40.9 \footnotesize{(0.96)} & 39.9 \footnotesize{(1.00)} & 38.7 \footnotesize{(1.00)} & 36.2 \footnotesize{(1.00)} \\
    & 512 & 39.6 \footnotesize{(0.99)} & 35.7 \footnotesize{(1.00)} & 37.6 \footnotesize{(1.00)} & 37.5 \footnotesize{(1.00)} \\
    & 768 & 36.5 \footnotesize{(1.00)} & 36.2 \footnotesize{(1.00)} & 36.1 \footnotesize{(1.00)} & 36.7 \footnotesize{(1.00)} \\
    & 1024 & 34.8 \footnotesize{(1.00)} & 28.2 \footnotesize{(1.00)} & 31.8 \footnotesize{(1.00)} & 32.0 \footnotesize{(1.00)} \\
    & 1200 & 34.0 \footnotesize{(0.98)} & 31.4 \footnotesize{(1.00)} & 33.1 \footnotesize{(1.00)} & 32.3 \footnotesize{(1.00)} \\
    & 1600 & 28.5 \footnotesize{(1.00)} & 31.2 \footnotesize{(1.00)} & 21.5 \footnotesize{(1.00)} & 27.1 \footnotesize{(1.00)} \\
    & 2048 & 15.4 \footnotesize{(1.00)} & 24.3 \footnotesize{(1.00)} & 22.2 \footnotesize{(1.00)} & 19.7 \footnotesize{(0.96)} \\
    \bottomrule
    \end{tabular}
    
    }
  % \caption{BLEU scores for \model{NLLB} (top) and \model{TowerBase} (bottom).}
  \caption{BLEU scores (and brevity penalty) for \model{NLLB200-distilled-600M} and \model{TowerBase-7b}.}
  
  \label{tab:res-base-bleu}
\end{table}

    % prompt Translate the following text from English into French.\textbackslash nEnglish SRC\textbackslash nFrench: TGT
    % \begin{tabular}{l|llll}
    % \toprule
    % $l_{max}$ & 2014 & 2015 & 2016 & 2017 \\
    % \midrule
    % sent & 41.9 \footnotesize{(1.00)} & 40.1 \footnotesize{(1.00)} & 38.0 \footnotesize{(1.00)} & 33.0 \footnotesize{(1.00)} \\
    % 256 & 40.5 \footnotesize{(1.00)} & 37.1 \footnotesize{(1.00)} & 38.3 \footnotesize{(1.00)} & 35.7 \footnotesize{(1.00)} \\
    % 512 & 37.6 \footnotesize{(1.00)} & 36.3 \footnotesize{(1.00)} & 37.4 \footnotesize{(1.00)} & 37.4 \footnotesize{(1.00)} \\
    % 768 & 32.1 \footnotesize{(1.00)} & 30.2 \footnotesize{(1.00)} & 35.8 \footnotesize{(1.00)} & 35.2 \footnotesize{(1.00)} \\
    % 1024 & 35.6 \footnotesize{(1.00)} & 36.6 \footnotesize{(1.00)} & 32.0 \footnotesize{(1.00)} & 29.4 \footnotesize{(1.00)} \\
    % 1200 & 35.9 \footnotesize{(0.97)} & 31.1 \footnotesize{(1.00)} & 33.9 \footnotesize{(1.00)} & 31.7 \footnotesize{(1.00)} \\
    % 1600 & 32.2 \footnotesize{(0.99)} & 29.6 \footnotesize{(1.00)} & 25.1 \footnotesize{(1.00)} & 27.6 \footnotesize{(1.00)} \\
    % 2048 & 24.9 \footnotesize{(0.99)} & 26.1 \footnotesize{(1.00)} & 18.9 \footnotesize{(1.00)} & 20.2 \footnotesize{(0.95)} \\
    % \bottomrule
    % \end{tabular}

==> tabs/vanilla-bleu/res-nllb-TED-distill-testsets-vanilla-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}
        \scalebox{0.72}{
    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 41.5 \footnotesize{(0.99)} & 40.1 \footnotesize{(1.00)} & 38.2 \footnotesize{(1.00)} & 38.3 \footnotesize{(1.00)} \\
     & Unif.\ & 37.0 \footnotesize{(0.96)} & 37.2 \footnotesize{(0.99)} & 35.6 \footnotesize{(1.00)} & 34.8 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 40.2 \footnotesize{(0.98)} & 39.5 \footnotesize{(1.00)} & 37.3 \footnotesize{(1.00)} & 37.2 \footnotesize{(1.00)} \\
     & Unif.\ & 39.4 \footnotesize{(0.98)} & 39.1 \footnotesize{(1.00)} & 37.2 \footnotesize{(1.00)} & 36.8 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 40.0 \footnotesize{(0.99)} & 39.6 \footnotesize{(1.00)} & 36.7 \footnotesize{(1.00)} & 36.3 \footnotesize{(1.00)} \\
     & Unif.\ & 40.7 \footnotesize{(0.99)} & 39.8 \footnotesize{(1.00)} & 37.5 \footnotesize{(1.00)} & 37.5 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 40.7 \footnotesize{(1.00)} & 39.7 \footnotesize{(1.00)} & 36.9 \footnotesize{(1.00)} & 36.5 \footnotesize{(1.00)} \\
     & Unif.\ & 41.0 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.00)} & 38.3 \footnotesize{(1.00)} & 38.0 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 39.2 \footnotesize{(0.96)} & 39.2 \footnotesize{(0.99)} & 36.6 \footnotesize{(1.00)} & 35.8 \footnotesize{(1.00)} \\
     & Unif.\ & 40.9 \footnotesize{(0.99)} & 41.1 \footnotesize{(1.00)} & 37.2 \footnotesize{(1.00)} & 37.8 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 33.0 \footnotesize{(0.88)} & 33.8 \footnotesize{(0.91)} & 31.2 \footnotesize{(0.92)} & 29.7 \footnotesize{(0.93)} \\
     & Unif.\ & 36.6 \footnotesize{(0.92)} & 39.7 \footnotesize{(0.99)} & 35.8 \footnotesize{(0.97)} & 34.9 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 23.8 \footnotesize{(0.77)} & 23.4 \footnotesize{(0.73)} & 23.7 \footnotesize{(0.82)} & 22.9 \footnotesize{(0.8)} \\
     & Unif.\ & 23.2 \footnotesize{(0.72)} & 24.6 \footnotesize{(0.82)} & 23.6 \footnotesize{(0.87)} & 25.7 \footnotesize{(0.83)} \\
      \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 19.4 \footnotesize{(0.66)} & 17.1 \footnotesize{(0.63)} & 20.1 \footnotesize{(0.74)} & 17.5 \footnotesize{(0.71)} \\
     & Unif.\ & 21.6 \footnotesize{(0.68)} & 19.0 \footnotesize{(0.61)} & 20.6 \footnotesize{(0.76)} & 18.0 \footnotesize{(0.68)} \\
     \bottomrule
    \end{tabular}
        }
 
    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}

    \scalebox{0.72}{

    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 84 & 85 & 85 & 84 \\
     & Unif.\ & 82 & 84 & 84 & 83 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 81 & 82 & 82 & 81 \\
     & Unif.\ & 81 & 82 & 82 & 81 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 81 & 82 & 81 & 80 \\
     & Unif.\ & 81 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 69 & 69 & 70 & 69 \\
     & Unif.\ & 74 & 75 & 74 & 73 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 58 & 59 & 60 & 58 \\
     & Unif.\ & 67 & 65 & 67 & 67 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 56 & 56 & 55 & 53 \\
     & Unif.\ & 61 & 65 & 62 & 60 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 50 & 49 & 49 & 49 \\
     & Unif.\ & 55 & 58 & 54 & 56 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 47 & 42 & 48 & 45 \\
     & Unif.\ & 51 & 49 & 51 & 48 \\
     \bottomrule
    \end{tabular}
}
    
    \caption{BLEU (left) and $100\times$COMET (right) scores for \FTnllbII (FT.\ ) and \UNIFnllbII (Unif.\ ) trained on \tedII with target max source document length $M=2048$.  }

    \label{tab:res-nllb-ted-distill-bleu-comet}
    \end{minipage}
\end{table*}



==> tabs/vanilla-bleu/res-nllb-TED-distill-testsets-vanilla-bleu.tex <==

\begin{table}
  \centering
    \scalebox{0.7}{
\begin{tabular}{llllll}
\toprule
 &  & 2014 & 2015 & 2016 & 2017 \\
 \midrule
\multirow[c]{2}{*}{sent} & FT.\ & 41.5 \footnotesize{(0.99)} & 40.1 \footnotesize{(1.0)} & 38.2 \footnotesize{(1.0)} & 38.3 \footnotesize{(1.0)} \\
 & Unif.\ & 37.0 \footnotesize{(0.96)} & 37.2 \footnotesize{(0.99)} & 35.6 \footnotesize{(1.0)} & 34.8 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{256} & FT.\ & 40.2 \footnotesize{(0.98)} & 39.5 \footnotesize{(1.0)} & 37.3 \footnotesize{(1.0)} & 37.2 \footnotesize{(1.0)} \\
 & Unif.\ & 39.4 \footnotesize{(0.98)} & 39.1 \footnotesize{(1.0)} & 37.2 \footnotesize{(1.0)} & 36.8 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{512} & FT.\ & 40.0 \footnotesize{(0.99)} & 39.6 \footnotesize{(1.0)} & 36.7 \footnotesize{(1.0)} & 36.3 \footnotesize{(1.0)} \\
 & Unif.\ & 40.7 \footnotesize{(0.99)} & 39.8 \footnotesize{(1.0)} & 37.5 \footnotesize{(1.0)} & 37.5 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{768} & FT.\ & 40.7 \footnotesize{(1.0)} & 39.7 \footnotesize{(1.0)} & 36.9 \footnotesize{(1.0)} & 36.5 \footnotesize{(1.0)} \\
 & Unif.\ & 41.0 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.0)} & 38.3 \footnotesize{(1.0)} & 38.0 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1024} & FT.\ & 39.2 \footnotesize{(0.96)} & 39.2 \footnotesize{(0.99)} & 36.6 \footnotesize{(1.0)} & 35.8 \footnotesize{(1.0)} \\
 & Unif.\ & 40.9 \footnotesize{(0.99)} & 41.1 \footnotesize{(1.0)} & 37.2 \footnotesize{(1.0)} & 37.8 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1200} & FT.\ & 33.0 \footnotesize{(0.88)} & 33.8 \footnotesize{(0.91)} & 31.2 \footnotesize{(0.92)} & 29.7 \footnotesize{(0.93)} \\
 & Unif.\ & 36.6 \footnotesize{(0.92)} & 39.7 \footnotesize{(0.99)} & 35.8 \footnotesize{(0.97)} & 34.9 \footnotesize{(1.0)} \\
  \midrule
\multirow[c]{2}{*}{1600} & FT.\ & 23.8 \footnotesize{(0.77)} & 23.4 \footnotesize{(0.73)} & 23.7 \footnotesize{(0.82)} & 22.9 \footnotesize{(0.8)} \\
 & Unif.\ & 23.2 \footnotesize{(0.72)} & 24.6 \footnotesize{(0.82)} & 23.6 \footnotesize{(0.87)} & 25.7 \footnotesize{(0.83)} \\
  \midrule
\multirow[c]{2}{*}{2048} & FT.\ & 19.4 \footnotesize{(0.66)} & 17.1 \footnotesize{(0.63)} & 20.1 \footnotesize{(0.74)} & 17.5 \footnotesize{(0.71)} \\
 & Unif.\ & 21.6 \footnotesize{(0.68)} & 19.0 \footnotesize{(0.61)} & 20.6 \footnotesize{(0.76)} & 18.0 \footnotesize{(0.68)} \\
 \bottomrule
\end{tabular}

    }
  \caption{BLEU for \FTnllbII (FT.\ ),  \UNIFnllbII (Unif.\ ) trained on \tedII with target max source document length 2048 }
  \label{tab:res-nllb-bleu-ted-distill}
\end{table}



==> tabs/vanilla-bleu/res-nllb-TED-unif-testsets-vanilla-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}

        \scalebox{0.72}{
    
    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 41.5 \footnotesize{(0.99)} & 40.1 \footnotesize{(1.00)} & 38.2 \footnotesize{(1.00)} & 38.3 \footnotesize{(1.00)} \\
     & Unif.\ & 37.0 \footnotesize{(0.96)} & 37.2 \footnotesize{(0.99)} & 35.6 \footnotesize{(1.00)} & 34.8 \footnotesize{(1.00)} \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 40.2 \footnotesize{(0.98)} & 39.5 \footnotesize{(1.00)} & 37.3 \footnotesize{(1.00)} & 37.2 \footnotesize{(1.00)} \\
     & Unif.\ & 39.4 \footnotesize{(0.98)} & 39.1 \footnotesize{(1.00)} & 37.2 \footnotesize{(1.00)} & 36.8 \footnotesize{(1.00)} \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 40.0 \footnotesize{(0.99)} & 39.6 \footnotesize{(1.00)} & 36.7 \footnotesize{(1.00)} & 36.3 \footnotesize{(1.00)} \\
     & Unif.\ & 40.7 \footnotesize{(0.99)} & 39.8 \footnotesize{(1.00)} & 37.5 \footnotesize{(1.00)} & 37.5 \footnotesize{(1.00)} \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 40.7 \footnotesize{(1.00)} & 39.7 \footnotesize{(1.00)} & 36.9 \footnotesize{(1.00)} & 36.5 \footnotesize{(1.00)} \\
     & Unif.\ & 41.0 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.00)} & 38.3 \footnotesize{(1.00)} & 38.0 \footnotesize{(1.00)} \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 39.2 \footnotesize{(0.96)} & 39.2 \footnotesize{(0.99)} & 36.6 \footnotesize{(1.00)} & 35.8 \footnotesize{(1.00)} \\
     & Unif.\ & 40.9 \footnotesize{(0.99)} & 41.1 \footnotesize{(1.00)} & 37.2 \footnotesize{(1.00)} & 37.8 \footnotesize{(1.00)} \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 33.0 \footnotesize{(0.88)} & 33.8 \footnotesize{(0.91)} & 31.2 \footnotesize{(0.92)} & 29.7 \footnotesize{(0.93)} \\
     & Unif.\ & 36.6 \footnotesize{(0.92)} & 39.7 \footnotesize{(0.99)} & 35.8 \footnotesize{(0.97)} & 34.9 \footnotesize{(1.00)} \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 23.8 \footnotesize{(0.77)} & 23.4 \footnotesize{(0.73)} & 23.7 \footnotesize{(0.82)} & 22.9 \footnotesize{(0.8)} \\
     & Unif.\ & 23.2 \footnotesize{(0.72)} & 24.6 \footnotesize{(0.82)} & 23.6 \footnotesize{(0.87)} & 25.7 \footnotesize{(0.83)} \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 19.4 \footnotesize{(0.66)} & 17.1 \footnotesize{(0.63)} & 20.1 \footnotesize{(0.74)} & 17.5 \footnotesize{(0.71)} \\
     & Unif.\ & 21.6 \footnotesize{(0.68)} & 19.0 \footnotesize{(0.61)} & 20.6 \footnotesize{(0.76)} & 18.0 \footnotesize{(0.68)} \\
     \bottomrule
    \end{tabular}

    }

    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}

    \scalebox{0.72}{
    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 84 & 85 & 85 & 84 \\
     & Unif.\ & 82 & 83 & 83 & 83 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 80 & 81 & 81 & 81 \\
     & Unif.\ & 80 & 81 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 80 & 81 & 81 & 81 \\
     & Unif.\ & 81 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 80 & 81 & 81 & 81 \\
     & Unif.\ & 81 & 82 & 82 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 78 & 79 & 78 & 78 \\
     & Unif.\ & 80 & 81 & 81 & 80 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 71 & 73 & 70 & 69 \\
     & Unif.\ & 76 & 79 & 76 & 75 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 61 & 60 & 61 & 60 \\
     & Unif.\ & 62 & 61 & 61 & 64 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 57 & 53 & 57 & 54 \\
     & Unif.\ & 59 & 57 & 57 & 54 \\
     \bottomrule
    \end{tabular}

}
    
    \caption{BLEU (left) and $100\times$COMET (right) scores for \FTnllbI (FT.\ ) and \UNIFnllbI (Unif.\ ) trained on \tedI with target max source document length $M=2048$.  }
    \label{tab:res-nllb-ted-unif-bleu-comet}
    \end{minipage}
\end{table*}



==> tabs/vanilla-bleu/res-nllb-TED-unif-testsets-vanilla-bleu.tex <==

\begin{table}
  \centering
    \scalebox{0.72}{
    
    \begin{tabular}{llllll}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 41.5 \footnotesize{(0.99)} & 40.1 \footnotesize{(1.0)} & 38.2 \footnotesize{(1.0)} & 38.3 \footnotesize{(1.0)} \\
     & Unif.\ & 37.0 \footnotesize{(0.96)} & 37.2 \footnotesize{(0.99)} & 35.6 \footnotesize{(1.0)} & 34.8 \footnotesize{(1.0)} \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 40.2 \footnotesize{(0.98)} & 39.5 \footnotesize{(1.0)} & 37.3 \footnotesize{(1.0)} & 37.2 \footnotesize{(1.0)} \\
     & Unif.\ & 39.4 \footnotesize{(0.98)} & 39.1 \footnotesize{(1.0)} & 37.2 \footnotesize{(1.0)} & 36.8 \footnotesize{(1.0)} \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 40.0 \footnotesize{(0.99)} & 39.6 \footnotesize{(1.0)} & 36.7 \footnotesize{(1.0)} & 36.3 \footnotesize{(1.0)} \\
     & Unif.\ & 40.7 \footnotesize{(0.99)} & 39.8 \footnotesize{(1.0)} & 37.5 \footnotesize{(1.0)} & 37.5 \footnotesize{(1.0)} \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 40.7 \footnotesize{(1.0)} & 39.7 \footnotesize{(1.0)} & 36.9 \footnotesize{(1.0)} & 36.5 \footnotesize{(1.0)} \\
     & Unif.\ & 41.0 \footnotesize{(0.99)} & 40.4 \footnotesize{(1.0)} & 38.3 \footnotesize{(1.0)} & 38.0 \footnotesize{(1.0)} \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 39.2 \footnotesize{(0.96)} & 39.2 \footnotesize{(0.99)} & 36.6 \footnotesize{(1.0)} & 35.8 \footnotesize{(1.0)} \\
     & Unif.\ & 40.9 \footnotesize{(0.99)} & 41.1 \footnotesize{(1.0)} & 37.2 \footnotesize{(1.0)} & 37.8 \footnotesize{(1.0)} \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 33.0 \footnotesize{(0.88)} & 33.8 \footnotesize{(0.91)} & 31.2 \footnotesize{(0.92)} & 29.7 \footnotesize{(0.93)} \\
     & Unif.\ & 36.6 \footnotesize{(0.92)} & 39.7 \footnotesize{(0.99)} & 35.8 \footnotesize{(0.97)} & 34.9 \footnotesize{(1.0)} \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 23.8 \footnotesize{(0.77)} & 23.4 \footnotesize{(0.73)} & 23.7 \footnotesize{(0.82)} & 22.9 \footnotesize{(0.8)} \\
     & Unif.\ & 23.2 \footnotesize{(0.72)} & 24.6 \footnotesize{(0.82)} & 23.6 \footnotesize{(0.87)} & 25.7 \footnotesize{(0.83)} \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 19.4 \footnotesize{(0.66)} & 17.1 \footnotesize{(0.63)} & 20.1 \footnotesize{(0.74)} & 17.5 \footnotesize{(0.71)} \\
     & Unif.\ & 21.6 \footnotesize{(0.68)} & 19.0 \footnotesize{(0.61)} & 20.6 \footnotesize{(0.76)} & 18.0 \footnotesize{(0.68)} \\
     \bottomrule
    \end{tabular}

    }
  \caption{BLEU for \FTnllbI (FT.\ ) and \UNIFnllbI (Unif.\ ) trained on \tedI with target max source document length 2048 }
  \label{ tab:res-nllb-bleu-ted-unif}
\end{table}



==> tabs/vanilla-bleu/res-tower-TED-distill-testsets-vanilla-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}

        \scalebox{0.72}{
        
    \begin{tabular}{ll|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 43.8 \footnotesize{(0.99)} & 41.7 \footnotesize{(1.00)} & 40.4 \footnotesize{(1.00)} & 36.8 \footnotesize{(1.00)} \\
     & Unif.\ & 43.8 \footnotesize{(0.99)} & 41.6 \footnotesize{(1.00)} & 40.4 \footnotesize{(1.00)} & 37.3 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 41.8 \footnotesize{(1.00)} & 41.5 \footnotesize{(1.00)} & 40.0 \footnotesize{(1.00)} & 38.8 \footnotesize{(1.00)} \\
     & Unif.\ & 41.6 \footnotesize{(1.00)} & 41.5 \footnotesize{(1.00)} & 40.0 \footnotesize{(1.00)} & 38.8 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 41.2 \footnotesize{(1.00)} & 41.5 \footnotesize{(1.00)} & 39.2 \footnotesize{(1.00)} & 38.5 \footnotesize{(1.00)} \\
     & Unif.\ & 41.1 \footnotesize{(1.00)} & 41.3 \footnotesize{(1.00)} & 39.2 \footnotesize{(1.00)} & 38.2 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 41.4 \footnotesize{(1.00)} & 40.9 \footnotesize{(1.00)} & 37.6 \footnotesize{(1.00)} & 37.6 \footnotesize{(1.00)} \\
     & Unif.\ & 41.4 \footnotesize{(1.00)} & 40.8 \footnotesize{(1.00)} & 37.5 \footnotesize{(1.00)} & 37.2 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 39.4 \footnotesize{(1.00)} & 36.4 \footnotesize{(1.00)} & 35.6 \footnotesize{(1.00)} & 37.1 \footnotesize{(1.00)} \\
     & Unif.\ & 39.2 \footnotesize{(1.00)} & 39.2 \footnotesize{(1.00)} & 36.5 \footnotesize{(1.00)} & 36.8 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 38.3 \footnotesize{(1.00)} & 39.7 \footnotesize{(1.00)} & 36.1 \footnotesize{(1.00)} & 37.4 \footnotesize{(1.00)} \\
     & Unif.\ & 38.3 \footnotesize{(1.00)} & 39.4 \footnotesize{(1.00)} & 36.5 \footnotesize{(1.00)} & 37.1 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 39.1 \footnotesize{(1.00)} & 37.7 \footnotesize{(1.00)} & 33.4 \footnotesize{(1.00)} & 35.1 \footnotesize{(1.00)} \\
     & Unif.\ & 39.3 \footnotesize{(1.00)} & 36.6 \footnotesize{(1.00)} & 34.0 \footnotesize{(1.00)} & 33.7 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 26.8 \footnotesize{(1.00)} & 27.6 \footnotesize{(1.00)} & 27.3 \footnotesize{(1.00)} & 24.7 \footnotesize{(1.00)} \\
     & Unif.\ & 27.4 \footnotesize{(1.00)} & 29.0 \footnotesize{(1.00)} & 28.8 \footnotesize{(1.00)} & 22.9 \footnotesize{(1.00)} \\
     \bottomrule
    \end{tabular}

    }


    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}
    
    \scalebox{0.72}{
    \begin{tabular}{ll|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 85 & 86 & 85 & 85 \\
     & Unif.\ & 85 & 86 & 85 & 85 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 83 & 84 & 83 & 83 \\
     & Unif.\ & 83 & 84 & 83 & 83 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 82 & 84 & 83 & 82 \\
     & Unif.\ & 82 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 82 & 83 & 83 & 82 \\
     & Unif.\ & 82 & 83 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 81 & 81 & 82 & 81 \\
     & Unif.\ & 81 & 82 & 83 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 78 & 82 & 81 & 81 \\
     & Unif.\ & 78 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 80 & 79 & 79 & 80 \\
     & Unif.\ & 79 & 78 & 79 & 78 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 68 & 69 & 68 & 64 \\
     & Unif.\ & 69 & 70 & 70 & 62 \\
     \bottomrule
    \end{tabular}
    }
    \caption{BLEU (left) and $100\times$COMET (right) scores for \FTtowerII (FT.\ ) and \UNIFtowerII (Unif-full) trained on \tedII with target max source document length 2048 ($M = 4096$).}
    \label{tab:res-tower-ted-distill-bleu-comet}
    \end{minipage}
\end{table*}



==> tabs/vanilla-bleu/res-tower-TED-unif-testsets-vanilla-BLEU-COMET.tex <==

\begin{table*} %[h]
    \centering
    \begin{minipage}{0.5\textwidth}

       \scalebox{0.72}{
    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 43.5 \footnotesize{(0.99)} & 41.8 \footnotesize{(1.00)} & 40.3 \footnotesize{(1.00)} & 36.7 \footnotesize{(1.00)} \\
     & Unif.\ & 43.6 \footnotesize{(0.99)} & 41.7 \footnotesize{(1.00)} & 40.4 \footnotesize{(1.00)} & 36.7 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 43.5 \footnotesize{(0.99)} & 41.5 \footnotesize{(1.00)} & 40.0 \footnotesize{(1.00)} & 38.7 \footnotesize{(1.00)} \\
     & Unif.\ & 41.8 \footnotesize{(1.00)} & 41.6 \footnotesize{(1.00)} & 40.1 \footnotesize{(1.00)} & 38.8 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 40.3 \footnotesize{(1.00)} & 41.5 \footnotesize{(1.00)} & 39.0 \footnotesize{(1.00)} & 38.3 \footnotesize{(1.00)} \\
     & Unif.\ & 38.9 \footnotesize{(1.00)} & 41.6 \footnotesize{(1.00)} & 39.2 \footnotesize{(1.00)} & 38.5 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 41.6 \footnotesize{(1.00)} & 41.1 \footnotesize{(1.00)} & 39.1 \footnotesize{(1.00)} & 37.6 \footnotesize{(1.00)} \\
     & Unif.\ & 40.4 \footnotesize{(1.00)} & 41.2 \footnotesize{(1.00)} & 39.3 \footnotesize{(1.00)} & 37.8 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 40.9 \footnotesize{(0.99)} & 37.7 \footnotesize{(1.00)} & 36.8 \footnotesize{(1.00)} & 36.4 \footnotesize{(1.00)} \\
     & Unif.\ & 39.6 \footnotesize{(1.00)} & 40.5 \footnotesize{(1.00)} & 36.8 \footnotesize{(1.00)} & 36.1 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 40.0 \footnotesize{(1.00)} & 39.5 \footnotesize{(1.00)} & 36.9 \footnotesize{(1.00)} & 37.5 \footnotesize{(1.00)} \\
     & Unif.\ & 39.7 \footnotesize{(1.00)} & 39.8 \footnotesize{(1.00)} & 35.9 \footnotesize{(1.00)} & 37.6 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 38.6 \footnotesize{(0.97)} & 37.4 \footnotesize{(1.00)} & 34.1 \footnotesize{(1.00)} & 36.4 \footnotesize{(1.00)} \\
     & Unif.\ & 38.4 \footnotesize{(1.00)} & 38.3 \footnotesize{(1.00)} & 32.9 \footnotesize{(1.00)} & 34.3 \footnotesize{(1.00)} \\
      \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 29.4 \footnotesize{(1.00)} & 31.3 \footnotesize{(1.00)} & 27.2 \footnotesize{(1.00)} & 25.3 \footnotesize{(1.00)} \\
     & Unif.\ & 30.0 \footnotesize{(1.00)} & 31.8 \footnotesize{(1.00)} & 26.4 \footnotesize{(1.00)} & 27.8 \footnotesize{(1.00)} \\
     \bottomrule
    \end{tabular}
    
    }



    \end{minipage}%
    \hspace{0.03\textwidth} % Space between tables
    \begin{minipage}{0.45\textwidth}

        \scalebox{0.72}{
    
    \begin{tabular}{rl|rrrr}
    \toprule
     &  & 2014 & 2015 & 2016 & 2017 \\
     \midrule
    \multirow[c]{2}{*}{sent} & FT.\ & 85 & 86 & 85 & 85 \\
     & Unif.\ & 85 & 86 & 85 & 85 \\
     \midrule
    \multirow[c]{2}{*}{256} & FT.\ & 83 & 84 & 83 & 83 \\
     & Unif.\ & 83 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{512} & FT.\ & 82 & 84 & 83 & 82 \\
     & Unif.\ & 82 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{768} & FT.\ & 82 & 83 & 83 & 82 \\
     & Unif.\ & 82 & 84 & 83 & 82 \\
     \midrule
    \multirow[c]{2}{*}{1024} & FT.\ & 81 & 81 & 83 & 81 \\
     & Unif.\ & 81 & 83 & 83 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1200} & FT.\ & 80 & 82 & 81 & 81 \\
     & Unif.\ & 80 & 82 & 81 & 81 \\
     \midrule
    \multirow[c]{2}{*}{1600} & FT.\ & 79 & 79 & 80 & 80 \\
     & Unif.\ & 80 & 80 & 78 & 79 \\
     \midrule
    \multirow[c]{2}{*}{2048} & FT.\ & 68 & 72 & 69 & 64 \\
     & Unif.\ & 70 & 72 & 69 & 67 \\

     \bottomrule
    \end{tabular}

    }

    
    \caption{BLEU (left) and $100\times$COMET (right) for \FTtowerI (FT.\ ) and \UNIFtowerI (Unif-full) trained on \tedI with target max source document length 2048 ($M = 4096$).}
    \label{tab:res-tower-ted-unif-bleu-comet}
    \end{minipage}
\end{table*}


